Optimal Myopic Attacks on Nonlinear Estimation

Recent high-profile incidents have exposed security risks in control systems. Particularly important and safety-critical modules for security analysis are estimation and control (E&C). Prior works have analyzed the security of E&C for linear, time-invariant systems; however, there are few analyses of nonlinear systems despite their broad use. In an effort to facilitate identifying vulnerabilities in control systems, in this work we establish a class of optimal attacks on nonlinear E&C. Specifically, we define two attack objectives and illustrate that realizing the optimal attacks against the widely-adopted extended Kalman filter with industry-standard $\chi^2$ anomaly detection is equivalent to solving convex quadratically-constrained quadratic programs. Given an appropriate information model for the attacker (i.e.,~a specified amount of attacker knowledge), we provide practical relaxations on the optimal attacks to allow for their computation at runtime. We also show that the difference between the optimal and relaxed attacks is bounded. Finally, we illustrate the use of the introduced attack designs on a case-study.

==> 99-extra.tex <==

\paragraph{Maximum-Deviation}
In a max-dev attack, the attacker wishes to cause the maximum deviation between the goal state and the true state in the L2-norm sense. However, that goal is difficult to formalize, particularly because: 1) the goal path should not rigidly depend on time since a change in traffic pattern (e.g.,~traffic jam) would be conflated with attack success, and 2) without a time-dependent goal path, only deviations lateral to the path would register successful, even though substantial deviation forward or backward can still be successful for the adversary (e.g.~rapid stopping on the freeway). As such, we instead consider that the attacker's goal should be to maximally deviate the navigator's state estimate from the true state under the belief that the control module will attempt to correct deviations in the estimated state from the goal state.


\paragraph{Direction-Conditional-Max-Deviation}
While a max-dev attack is indifferent to the direction of deviation, a direction-conditional max-dev attack desires to deviate the platform in an attacker-specified direction. This formulation requires only two changes relative to the max-dev attack.

First, the notion of a rotational basis must be identified to define directions. The naive approach of defining the direction by the AV's current elocity vector is undesirable in most cases with physical actuation limitations (e.g.,~turning a car "left" would constantly change the basis and would lead to circular motion). Instead, we define the basis where the x-axis is in the direction of travel along the guidance path, the z-axis is anti-parallel to the gravity gradient, and the y-axis completes a right-handed system (notionally, "left"). We define "forward" by taking the closest point on the guidance path from the true state in the L2-sense and pointing in the desired direction of travel (to the next point in $p^*$). This may have discontinuities, say when the guidance path follows a gradual turn but the AV sharply cuts the turn. However, forcing the AV to sharply cut the turn enough to make the guidance path discontinuous would represent great success on behalf of the adversary, so we do not bother to address this.

Second, the notion of directions must be formalized. We formalize the problem by defining a desired deviation direction and transforming that direction into the rotational basis. When empirically testing the direction-conditional attack, we limit to only considering deviation along the planar basis vectors (i.e.,~forward, backward, left, and right), as we find it easier to visualize and interpret the results.

Thus, the direction-conditional max-dev attack becomes
\begin{align} \label{eq:goal-dir-cond-max-dev}
    \max_a \ \bm{d}_g^T \, \cdot R_w^g \, \cdot C \cdot (x_k - \hat{x}_{k|k})
\end{align}
in the one-step case, where $\bm{d}_g$ is the unit vector defining the desired direction of deviation and $R_w^g$ is the transformation from world coordinates to the local coordinates of the closest point (defined by $p^*$ and $x_k$) on the guidance path.




\paragraph{Take-To-Point}
We finally consider a challenging attack goal where the adversary wants to take the attacker as close as possible to an adversary-specified state in world coordinates as quickly as possible. This attack formalizes as


which is best understood as: design attacks to bring the agent to within a threshold, $\delta$, of the adversary's goal state, $\mathcal{X}^a$, as fast as possible.

In the remainder of this work, we explore the case where $C$ is defined to pull out position states.









 
All cases specify the attack goal as depending on the true state of the AV. When it is necessary to directly evaluate the goal equation (e.g.,~in direct optimization), we must make an approximation to the true state. With different levels of knowledge, this approximation will have differing degrees of accuracy. In all cases, we represent the agent's estimate of the true state as $\mathring{\hat{x}}_{k|k}$.


% ======
\paragraph{Reinforcement Learning}
To fit into the RL framework, we can formulate the objective as an MDP where the agent wants to take actions (add attack bias) to increase the true state's deviation. To have enough information to learn actions according to equation~\ref{eq:nav-knowledge-max-dev}, the agent's MDP state must contain information on: 1) the agent's estimate of the navigation state $\mathring{\hat{x}}_{k|k}$, 2) the navigator's predicted estimate of the nav state $\hat{x}_{k|k-1}$, 3) the incoming measurements $z_k$, and 4) the matrices $P_{k|k-1}$, $H_k$, and $R_k$. We can make the simplifying assumption that, since we just care about GNSS, $H_k$ is always identity in position and that $R_k$ is a diagonal matrix where the measurement noise entries are all $\rho$, i.e.~the same across each axis, although these assumptions are not strictly necessary to solve the problem.

Since the estimation problem is shift and scale-invariant, we can shift our vector quantities to have origin at the incoming measurements and scale Cartesian quantities to make $\rho=1$ on each frame using a scaling-vector~$\xi$. Furthermore, if $\mathring{\hat{x}}_{k|k}$ has an angle estimate, we can rotate coordinates of $\mathring{\hat{x}}_{k|k}$, $\hat{x}_{k|k-1}$, and $P_{k|k-1}$ into the estimated body frame using a rotation matrix~$R_w^b$ built from the attitude state estimate. Thus, we have new vector and matrix quantities:

\begin{align}
    \mathring{\hat{v}}_{k|k} \coloneqq  \xi \odot \left( 
    \mathring{\hat{x}}_{k|k} - \begin{bmatrix}
        z_k\\
        \boldsymbol{0}
    \end{bmatrix} \right)\\
    \hat{v}_{k|k-1} \coloneqq \xi \odot \left(
    \hat{x}_{k|k-1}- \begin{bmatrix}
        z_k\\
        \boldsymbol{0}
    \end{bmatrix} \right)\\
    \mathcal{P}_{k|k-1} \coloneqq P_{k|k-1} \odot \left( \xi \xi^T \right)
\end{align}
where we make the following definitions
\begin{align*}
    R_w^b \coloneqq \text{Rotation from world to } \mathring{\hat{x}}_{k|k-1} \text{ body}\\
    \xi \coloneqq \begin{bmatrix} \xi_1, \ldots, \xi_n \end{bmatrix}^T \text{where } \xi_i \coloneqq \begin{cases}
    \sfrac{1}{\rho}, & \text{if } i \in \mathcal{C}\\
    1, & \text{otherwise}
    \end{cases}\\
    \mathcal{C} \coloneqq \{i \ | \ i \text{ is index of a Cartesian state}\}
\end{align*}
with an $n$-dimensional state where we typically have the first elements as position for the navigation problem. We abuse notation slightly here for simplicity by writing the rotation operation on $\hat{v}_{k|k-1}$ attitude as a matrix-vector product. Note that the attitude angles of $\mathring{\hat{v}}_{k|k}$ are always 0 in its own body frame.

Formally, the MDP becomes:
\begin{itemize}
    \item States: ($R_w^b\mathring{\hat{v}}_{k|k}$, $R_w^b\hat{v}_{k|k-1}$, $R_w^b\mathcal{P}_{k|k-1}(R_w^b)^T$)
    \vspace{-4pt}
    \item Actions: $a_k$ attack biases - after rescaling by $\rho$, rotating by $(R_w^b)^T$
    \vspace{-4pt}
    \item Transition Function: The true state is actuated by control signals sent from the control module which minimizes a notion of difference between $\hat{x}_{k|k}(a_k)$ (defined in equation~\ref{eq:nav-knowledge-max-dev}) and the goal path, $p^*$.
    \vspace{-4pt}
    \item Rewards: Agent receives a reward based on the incremental deviation of the navigator's estimated state from the true state $x_k$. Agent also receives a negative reward if the attacked measurement violates the $\chi^2$ integrity test.
    \vspace{-4pt}
    \begin{align}
        \begin{split}
            \Phi(s_i) &= \|Cx_{i} - C\hat{x}_{i|i}\|\\
            R_{1}(s_{k-1},a,s_k) &= \Phi(s_k) - \Phi(s_{k-1})\\
            R_{2}(s_{k-1},a,s_k) &= \begin{cases}
            -\beta & \text{if} \ y(a_k)^T S_k^{-1} y(a_k) > \tau\\
            0 & \text{otherwise}
            \end{cases}\\
            R &= R_1 + R_2
        \end{split}
    \end{align}
\end{itemize}


% ======
\paragraph{Reinforcement Learning}
There are only two modifications over the max-dev formulation that need be made for this MDP: augmenting both the state and rewards with a notion of the conditioned goal. Instead of rotating states into the local body frame, we transform them into the estimated guidance frame and we provide the agent a reward based on the deviation projected along the goal direction.

To reduce model complexity, we train and deploy separate agents for each of the allowed directions (i.e.~one for each of forward, backward, left, and right). That way, the conditioned goal need not be added to the state - only executed in the reward function for each sub-network. 

\begin{enumerate}
    \item States: \\($\hat{R}_{w,k}^g\mathring{\hat{v}}_{k|k}$, $\hat{R}_{w,k}^g\hat{v}_{k|k-1}$, $\hat{R}_{w,k}^g\mathcal{P}_{k|k-1}(\hat{R}_{w,k}^g)^T$)
    \item Actions: $a_k$ attack biases - after rescaling by $\rho$, rotating by $(R_{w,k}^g)^T$
    \item Transition Function: control signal actuation, subsequent AV movement, and sensor measurements
    \item Rewards: incremental deviation along the goal-conditioned direction
    \begin{align}
        \begin{split}
            \Phi(s_i) &= \bm{d}_g^T \, \cdot R_{w,i}^g \, \cdot C \cdot (x_i - \hat{x}_{i|i})\\
            R_{1}(s_{k-1},a,s_k) &= \Phi(s_k) - \Phi(s_{k-1})\\
            R_{2}(s_{k-1},a,s_k) &= \begin{cases}
            -\beta & \text{if} \ y(a_k)^T S_k^{-1} y(a_k) > \tau\\
            0 & \text{otherwise}
            \end{cases}\\
            R &= R_1 + R_2
        \end{split}
    \end{align}
\end{enumerate}
% ======
\paragraph{Reinforcement Learning}
The MDP formulation only requires simple modifications of the max-dev case. We can augment the state with the shifted and scaled goal state
\begin{align}
    \mathcal{\check{X}}^a \coloneqq \xi \odot \left( \mathcal{X}^a - \begin{bmatrix}
        z_k\\
        \boldsymbol{0}
    \end{bmatrix} \right)
\end{align}
and update the reward function to match the problem.

Formally, the MDP becomes:
\begin{itemize}
    \item States:\\($\hat{R}_w^b\mathring{\hat{v}}_{k|k}$, $\hat{R}_w^b\hat{v}_{k|k-1}$, $\hat{R}_w^b\mathcal{P}_{k|k-1}(\hat{R}_w^b)^T$, $\hat{R}_w^b\,\mathcal{\check{X}}^a$)
    \vspace{-4pt}
    \item Actions: $a_k$ attack biases - after rescaling by $\rho$, rotating by $(\hat{R}_{w,k}^g)^T$
    \vspace{-4pt}
    \item Transition Function: control signal actuation, subsequent AV movement, and sensor measurements
    \vspace{-4pt}
    \item Rewards: composed of base rewards ($R$) and shaping rewards ($W$) and total reward is $R + \beta W$\\
    \vspace{-4pt}
    \begin{align}
        \begin{split}
            R_1(s_{k-1},a,s_{k}) &= \begin{cases}
            \alpha, & \text{if} \ \|\mathcal{X}^a - C x_k\| \leq \delta\\
            0, & \text{otherwise}
            \end{cases}\\
            R_{2}(s_{k-1},a,s_k) &= \begin{cases}
                -\beta & \text{if} \ y(a_k)^T S_k^{-1} y(a_k) > \tau\\
                0 & \text{otherwise}
            \end{cases}\\
            R &= R_1 + R_2
        \end{split}
    \end{align}
    \begin{align}
        \begin{split}
            \Phi(s_i) = \|\mathcal{X}^a - C x_i\| \\
            W(s_{k-1},a,s_k) = \Phi(s_k) - \Phi(s_{k-1}) \\
        \end{split}
    \end{align}
    with $\delta$ a threshold to denote success of the episode. 
\end{itemize}

==> references_ALL.tex <==
@article{Liu2021,
    title = {{" Seeing is not Always Believing": Detecting Perception Error Attacks Against Autonomous Vehicles}},
    year = {2021},
    journal = {IEEE Transactions on Dependable and Secure Computing},
    author = {Liu, Jinshan and Park, Jerry},
    publisher = {IEEE},
    issn = {1545-5971}
}

@misc{Cao2020,
    title = {{3D adversarial object against msf-based perception in autonomous driving}},
    year = {2020},
    author = {Cao, Yulong and Wang, Ningfei and Xiao, Chaowei and Yang, Dawei and Fang, Jin and Yang, Ruigang and Chen, Qi Alfred and Liu, Mingyan and Li, Bo},
    publisher = {MLSys}
}

@inproceedings{Mousavian2017,
    title = {{3d bounding box estimation using deep learning and geometry}},
    year = {2017},
    booktitle = {Proceedings of the IEEE conference on Computer Vision and Pattern Recognition},
    author = {Mousavian, Arsalan and Anguelov, Dragomir and Flynn, John and Kosecka, Jana},
    pages = {7074--7082}
}

@inproceedings{Chen2015,
    title = {{3d object proposals for accurate object class detection}},
    year = {2015},
    booktitle = {Advances in Neural Information Processing Systems},
    author = {Chen, Xiaozhi and Kundu, Kaustav and Zhu, Yukun and Berneshawi, Andrew G and Ma, Huimin and Fidler, Sanja and Urtasun, Raquel},
    pages = {424--432},
    publisher = {Citeseer}
}

@article{Smith2011a,
    title = {{A decoupled feedback structure for covertly appropriating networked control systems}},
    year = {2011},
    journal = {IFAC Proceedings Volumes (IFAC-PapersOnline)},
    author = {Smith, Roy S.},
    number = {1 PART 1},
    pages = {90--95},
    volume = {44},
    publisher = {Elsevier},
    isbn = {9783902661937},
    doi = {10.3182/20110828-6-IT-1002.01721},
    issn = {14746670}
}

@article{Schoettle2015,
    title = {{A preliminary analysis of real-world crashes involving self-driving vehicles}},
    year = {2015},
    journal = {University of Michigan Transportation Research Institute},
    author = {Schoettle, Brandon and Sivak, Michael}
}

@article{Ding2018a,
    title = {{A survey on security control and attack detection for industrial cyber-physical systems}},
    year = {2018},
    journal = {Neurocomputing},
    author = {Ding, Derui and Han, Qing Long and Xiang, Yang and Ge, Xiaohua and Zhang, Xian Ming},
    pages = {1674--1683},
    volume = {275},
    publisher = {Elsevier},
    doi = {10.1016/j.neucom.2017.10.009},
    issn = {18728286},
    keywords = {Attack detection, Cyber-attacks, Industrial cyber-physical systems, Security control}
}

@article{Recht2019,
    title = {{A tour of reinforcement learning: The view from continuous control}},
    year = {2018},
    journal = {arXiv},
    author = {Recht, Benjamin},
    pages = {253--279},
    volume = {2},
    publisher = {Annual Reviews},
    doi = {10.1146/annurev-control-053018-023825},
    issn = {23318422},
    arxivId = {1806.09460}
}

@inproceedings{Anderson2005c,
    title = {{Active learning for hidden markov models: Objective functions and algorithms}},
    year = {2005},
    booktitle = {ICML 2005 - Proceedings of the 22nd International Conference on Machine Learning},
    author = {Anderson, Brigham and Moore, Andrew},
    pages = {9--16},
    isbn = {1595931805}
}

@inproceedings{Buisson-Fenet2020a,
    title = {{Actively learning Gaussian process dynamics}},
    year = {2019},
    booktitle = {arXiv},
    author = {Buisson-Fenet, Mona and Solowjow, Friedrich and Trimpe, Sebastian},
    pages = {5--15},
    publisher = {PMLR},
    isbn = {2640-3498},
    issn = {23318422},
    arxivId = {1911.09946},
    keywords = {Active learning, Gaussian process regression, Nonlinear system identification}
}

@article{Yang2019b,
    title = {{Adversarial Attack and Defense on Point Sets}},
    year = {2019},
    journal = {arXiv preprint arXiv:1902.10899},
    author = {Zhang, Qiang and Yang, Jiancheng and Fang, Rongyao and Ni, Bingbing and Liu, Jinxian and Tian, Qi},
    url = {http://arxiv.org/abs/1902.10899},
    arxivId = {1902.10899}
}

@inproceedings{Zeng2017,
    title = {{Adversarial attacks beyond the image space}},
    year = {2017},
    booktitle = {arXiv},
    author = {Zeng, Xiaohui and Liu, Chenxi and Wang, Yu Siang and Qiu, Weichao and Xie, Lingxi and Tai, Yu Wing and Tang, Chi Keung and Yuille, Alan L.},
    pages = {4302--4311},
    issn = {23318422}
}

@article{Abdelfattah2021,
    title = {{Adversarial Attacks on Camera-LiDAR Models for 3D Car Detection}},
    year = {2021},
    journal = {arXiv preprint arXiv:2103.09448},
    author = {Abdelfattah, Mazen and Yuan, Kaiwen and Wang, Z Jane and Ward, Rabab}
}

@inproceedings{Carlini2017e,
    title = {{Adversarial examples are not easily detected: Bypassing ten detection methods}},
    year = {2017},
    booktitle = {AISec 2017 - Proceedings of the 10th ACM Workshop on Artificial Intelligence and Security, co-located with CCS 2017},
    author = {Carlini, Nicholas and Wagner, David},
    pages = {3--14},
    isbn = {9781450352024},
    doi = {10.1145/3128572.3140444},
    arxivId = {1705.07263}
}

@inproceedings{Xie2017a,
    title = {{Adversarial examples for semantic segmentation and object detection}},
    year = {2017},
    booktitle = {arXiv},
    author = {Xie, Cihang and Wang, Jianyu and Zhang, Zhishuai and Zhou, Yuyin and Xie, Lingxi and Yuille, Alan},
    pages = {1369--1378},
    issn = {23318422}
}

@misc{Kurakin2016a,
    title = {{Adversarial examples in the physical world}},
    year = {2019},
    booktitle = {5th International Conference on Learning Representations, ICLR 2017 - Workshop Track Proceedings},
    author = {Kurakin, Alexey and Goodfellow, Ian J. and Bengio, Samy},
    doi = {10.1201/9781351251389-8},
    arxivId = {1607.02533}
}

@article{Lu2017,
    title = {{Adversarial examples that fool detectors}},
    year = {2017},
    journal = {arXiv},
    author = {Lu, Jiajun and Sibai, Hussein and Fabry, Evan},
    issn = {23318422},
    arxivId = {1712.02494}
}

@article{Brown2017,
    title = {{Adversarial patch}},
    year = {2017},
    journal = {arXiv preprint arXiv:1712.09665},
    author = {Brown, Tom B and Man{\'{e}}, Dandelion and Roy, Aurko and Abadi, Martín and Gilmer, Justin}
}

@article{Fischer2018b,
    title = {{Adversarial resilience learning - Towards systemic vulnerability analysis for large and complex systems}},
    year = {2018},
    journal = {arXiv},
    author = {Fischer, Lars and Memmen, Jan Menno and Veith, Eric Msp and Tr{\"{o}}schel, Martin},
    issn = {23318422},
    arxivId = {1811.06447},
    keywords = {Adversarial control, Power grid, Reinforcement learning, Resilience}
}

@inproceedings{Cao2019d,
    title = {{Adversarial sensor attack on lidar-based perception in autonomous driving}},
    year = {2019},
    booktitle = {Proceedings of the 2019 ACM SIGSAC conference on computer and communications security},
    author = {Cao, Yulong and Xiao, Chaowei and Cyr, Benjamin and Zhou, Yimeng and Park, Won and Rampazzi, Sara and Chen, Qi Alfred and Fu, Kevin and Mao, Z Morley},
    pages = {2267--2281},
    issn = {23318422},
    keywords = {Adversarial machine learning, Autonomous driving, Sensor attack}
}

@article{Shafahi2019,
    title = {{Adversarial Training for Free!}},
    year = {2019},
    journal = {arXiv},
    author = {Shafahi, Ali and Najibi, Mahyar and Ghiasi, Amin and Xu, Zheng and Dickerson, John and Davis, Larry S. and Goldstein, Tom and Studer, Christoph and Taylor, Gavin},
    issn = {23318422},
    arxivId = {1904.12843}
}

@inproceedings{Hamdi2020b,
    title = {{AdvPC: Transferable adversarial perturbations on 3D point clouds}},
    year = {2019},
    booktitle = {arXiv},
    author = {Hamdi, Abdullah and Rojas, Sara and Thabet, Ali and Ghanem, Bernard},
    pages = {241--257},
    publisher = {Springer},
    issn = {23318422}
}

@article{Wang2021a,
    title = {{AdvSim: Generating Safety-Critical Scenarios for Self-Driving Vehicles}},
    year = {2021},
    journal = {arXiv preprint arXiv:2101.06549},
    author = {Wang, Jingkang and Pun, Ava and Tu, James and Manivasagam, Sivabalan and Sadat, Abbas and Casas, Sergio and Ren, Mengye and Urtasun, Raquel}
}

@article{Szepesvari2010,
    title = {{Algorithms for reinforcement learning}},
    year = {2010},
    journal = {Synthesis Lectures on Artificial Intelligence and Machine Learning},
    author = {Szepesv{\'{a}}ri, Csaba},
    number = {1},
    pages = {1--89},
    volume = {9},
    publisher = {Morgan {\&} Claypool Publishers},
    isbn = {9781608454921},
    doi = {10.2200/S00268ED1V01Y201005AIM009},
    issn = {19394608},
    keywords = {Markov Decision Processes, Monte-Carlo methods, PAC-learning, Q-learning, active learning, actor-critic methods, bias-variance tradeoff, function approximation, least-squares methods, natural gradient, online learning, overfitting, planning, policy gradient, reinforcement learning, simulation, simulation optimization, stochastic approximation, stochastic gradient methods, temporal difference learning, two-timescale stochastic approximation}
}

@inproceedings{Moosavi-Dezfooli2017,
    title = {{Analysis of universal adversarial perturbations}},
    year = {2017},
    booktitle = {arXiv},
    author = {Moosavi-Dezfooli, Seyed Mohsen and Fawzi, Alhussein and Fawzi, Omar and Frossard, Pascal and Soatto, Stefano},
    pages = {1765--1773},
    issn = {23318422}
}

@inproceedings{Mnih2016b,
    title = {{Asynchronous methods for deep reinforcement learning}},
    year = {2016},
    booktitle = {33rd International Conference on Machine Learning, ICML 2016},
    author = {Mnih, Volodymyr and Badia, Adria Puigdomenech and Mirza, Lehdi and Graves, Alex and Harley, Tim and Lillicrap, Timothy P. and Silver, David and Kavukcuoglu, Koray},
    pages = {2850--2869},
    volume = {4},
    isbn = {9781510829008},
    arxivId = {1602.01783}
}

@article{Pasqualetti2012b,
    title = {{Attack detection and identification in cyber-physical systems}},
    year = {2013},
    journal = {IEEE Transactions on Automatic Control},
    author = {Pasqualetti, Fabio and Dorfler, Florian and Bullo, Francesco},
    number = {11},
    pages = {2715--2729},
    volume = {58},
    doi = {10.1109/TAC.2013.2266831},
    issn = {00189286},
    keywords = {Cyber-physical systems, descriptor systems, distributed control, fault detection, geometric control, graph theory, networks, security}
}

@article{Pasqualetti2013a,
    title = {{Attack detection and identification in cyber-physical systems}},
    year = {2013},
    journal = {IEEE Transactions on Automatic Control},
    author = {Pasqualetti, Fabio and Dorfler, Florian and Bullo, Francesco},
    number = {11},
    pages = {2715--2729},
    volume = {58},
    publisher = {IEEE},
    doi = {10.1109/TAC.2013.2266831},
    issn = {00189286},
    keywords = {Cyber-physical systems, descriptor systems, distributed control, fault detection, geometric control, graph theory, networks, security}
}

@inproceedings{Ivanov2014b,
    title = {{Attack-resilient sensor fusion}},
    year = {2014},
    booktitle = {2014 Design, Automation {\&} Test in Europe Conference {\&} Exhibition (DATE)},
    author = {Ivanov, Radoslav and Pajic, Miroslav and Lee, Insup},
    pages = {1--6},
    publisher = {IEEE},
    isbn = {3981537025}
}

@article{Pajic2016b,
    title = {{Attack-resilient state estimation for noisy dynamical systems}},
    year = {2017},
    journal = {IEEE Transactions on Control of Network Systems},
    author = {Pajic, Miroslav and Lee, Insup and Pappas, George J.},
    number = {1},
    pages = {82--92},
    volume = {4},
    publisher = {IEEE},
    doi = {10.1109/TCNS.2016.2607420},
    issn = {23255870},
    keywords = {Attack-resilient state estimation, cyberphysical systems security, linear systems, robustness of state estimators}
}

@article{Khazraei2020a,
    title = {{Attack-Resilient State Estimation with Intermittent Data Authentication}},
    year = {2020},
    journal = {arXiv},
    author = {Khazraei, Amir and Pajic, Miroslav},
    issn = {23318422},
    arxivId = {2005.08122},
    keywords = {Attack-resilient state estimation, Cyber-physical systems, Perfect attackability, Security of control systems}
}

@inproceedings{Wang2019,
    title = {{Attacking graph-based classification via manipulating the graph structure}},
    year = {2019},
    booktitle = {arXiv},
    author = {Wang, Binghui and Gong, Neil Zhenqiang},
    pages = {2023--2040},
    issn = {23318422},
    keywords = {Adversarial graph neural network, Adversarial graph-based classification, Adversarial machine learning}
}

@article{Boloor2020b,
    title = {{Attacking vision-based perception in end-to-end autonomous driving models}},
    year = {2019},
    journal = {Journal of Systems Architecture},
    author = {Boloor, Adith and Garimella, Karthik and He, Xin and Gill, Christopher and Vorobeychik, Yevgeniy and Zhang, Xuan},
    pages = {101766},
    volume = {110},
    publisher = {Elsevier},
    issn = {23318422},
    arxivId = {1910.01907},
    keywords = {Adversarial examples, Autonomous driving, Bayesian optimization, End-to-end learning, Machine learning}
}

@inproceedings{Kutila2016,
    title = {{Automotive LIDAR sensor development scenarios for harsh weather conditions}},
    year = {2016},
    booktitle = {2016 IEEE 19th International Conference on Intelligent Transportation Systems (ITSC)},
    author = {Kutila, Matti and Pyyk{\"{o}}nen, Pasi and Ritter, Werner and Sawade, Oliver and Sch{\"{a}}ufele, Bernd},
    pages = {265--270},
    publisher = {IEEE},
    isbn = {1509018891}
}

@inproceedings{Kim2004a,
    title = {{Autonomous helicopter flight via reinforcement learning}},
    year = {2004},
    booktitle = {Advances in Neural Information Processing Systems},
    author = {Ng, Andrew Y. and Kim, H. Jin and Jordan, Michael I. and Sastry, Shankar},
    pages = {799--806},
    isbn = {0262201526},
    doi = {10.1007/978-0-387-30164-8{\_}45},
    issn = {10495258}
}

@article{VanBrummelen2018,
    title = {{Autonomous vehicle perception: The technology of today and tomorrow}},
    year = {2018},
    journal = {Transportation research part C: emerging technologies},
    author = {Van Brummelen, Jessica and O’Brien, Marie and Gruyer, Dominique and Najjaran, Homayoun},
    pages = {384--406},
    volume = {89},
    publisher = {Elsevier},
    issn = {0968-090X}
}

@inproceedings{Thing2016,
    title = {{Autonomous vehicle security: A taxonomy of attacks and defences}},
    year = {2016},
    booktitle = {2016 ieee international conference on internet of things (ithings) and ieee green computing and communications (greencom) and ieee cyber, physical and social computing (cpscom) and ieee smart data (smartdata)},
    author = {Thing, Vrizlynn L L and Wu, Jiaxi},
    pages = {164--170},
    publisher = {IEEE},
    isbn = {150905880X}
}

@inproceedings{Hong2020,
    title = {{AVGuardian: Detecting and Mitigating Publish-Subscribe Overprivilege for Autonomous Vehicle Systems}},
    year = {2020},
    booktitle = {2020 IEEE European Symposium on Security and Privacy (EuroS{\&}P)},
    author = {Hong, David Ke and Kloosterman, John and Jin, Yuqi and Cao, Yulong and Chen, Qi Alfred and Mahlke, Scott and Mao, Z Morley},
    pages = {445--459},
    publisher = {IEEE},
    isbn = {1728150876}
}

@inproceedings{Pham2019,
    title = {{A∗3D Dataset: Towards Autonomous Driving in Challenging Environments}},
    year = {2019},
    booktitle = {arXiv},
    author = {Pham, Quang Hieu and Sevestre, Pierre and Pahwa, Ramanpreet Singh and Zhan, Huijing and Pang, Chun Ho and Chen, Yuda and Mustafa, Armin and Chandrasekhar, Vijay and Lin, Jie},
    pages = {2267--2273},
    publisher = {IEEE},
    isbn = {1728173957},
    issn = {23318422}
}

@article{Gu2019,
    title = {{BadNets: Evaluating Backdooring Attacks on Deep Neural Networks}},
    year = {2019},
    journal = {IEEE Access},
    author = {Gu, T and Liu, K and Dolan-Gavitt, B and Garg, S},
    pages = {47230--47244},
    volume = {7},
    doi = {10.1109/ACCESS.2019.2909068},
    issn = {2169-3536 VO  - 7},
    keywords = {BadNet, Biological neural networks, Computational modeling, Computer security, Machine learning, Perturbation methods, Security, Training, backdoor trigger, backdoored handwritten digit classifier, backdoored neural network, backdooring attack evaluation, deep learning-based techniques, deep neural networks, feedforward neural nets, learning (artificial intelligence), machine learning, maliciously trained network, neural networks, outsourced training, outsourcing, pattern classification, pre-trained models, security risks, specific attacker-chosen inputs, stop sign, street sign classifier, street sign detector, training procedure}
}

@article{Gu2017,
    title = {{Badnets: Identifying vulnerabilities in the machine learning model supply chain}},
    year = {2017},
    journal = {arXiv},
    author = {Gu, Tianyu and Dolan-Gavitt, Brendan and Garg, Siddharth},
    issn = {23318422},
    arxivId = {1708.06733}
}

@article{Charniak1991,
    title = {{Bayesian networks without tears}},
    year = {1991},
    journal = {AI Magazine},
    author = {Charniak, Eugene},
    number = {4},
    pages = {50--63},
    volume = {12},
    issn = {07384602}
}

@article{Chen2021a,
    title = {{Camdar-adv: Generating adversarial patches on 3D object}},
    year = {2021},
    journal = {International Journal of Intelligent Systems},
    author = {Chen, Chang and Huang, Teng},
    number = {3},
    pages = {1441--1453},
    volume = {36},
    publisher = {Wiley Online Library},
    doi = {10.1002/int.22349},
    issn = {1098111X},
    keywords = {Adversarial example, autonmous driving, geometric transformation}
}

@inproceedings{Barreno2006b,
    title = {{Can machine learning be secure?}},
    year = {2006},
    booktitle = {Proceedings of the 2006 ACM Symposium on Information, Computer and Communications Security, ASIACCS '06},
    author = {Barreno, Marco and Nelson, Blaine and Sears, Russell and Joseph, Anthony D. and Tygar, J. D.},
    pages = {16--25},
    volume = {2006},
    isbn = {1595932720},
    doi = {10.1145/1128817.1128824},
    keywords = {Adversarial learning, Computer networks, Computer security, Game theory, Intrusion detection, Machine learning, Security metrics, Spam filters, Statistical learning}
}

@article{Goodall2016,
    title = {{Can you program ethics into a self-driving car?}},
    year = {2016},
    journal = {IEEE Spectrum},
    author = {Goodall, Noah J},
    number = {6},
    pages = {28--58},
    volume = {53},
    publisher = {IEEE},
    issn = {0018-9235}
}

@article{Yan2016b,
    title = {{Can You Trust Autonomous Vehicles: Contactless Attacks against Sensors of Self-Driving Vehicles}},
    year = {2016},
    journal = {Def Con 24},
    author = {Yan, Chen and Xu, Wenyuan and Liu, Jianhao and 360, Qihoo},
    number = {8},
    pages = {109},
    volume = {24},
    url = {https://media.defcon.org/DEF CON 24/DEF CON 24 presentations/DEFCON-24-Liu-Yan-Xu-Can-You-Trust-Autonomous-Vehicles-WP.pdf},
    isbn = {9781450321389},
    doi = {10.1145/1235},
    issn = {16130073},
    arxivId = {arXiv:1603.07016v1},
    keywords = {Autonomous vehicles, cameras, millimeter-wave radars, security, ultrasonic sensors}
}

@inproceedings{Cohen2019b,
    title = {{Certified adversarial robustness via randomized smoothing}},
    year = {2019},
    booktitle = {arXiv},
    author = {Cohen, Jeremy and Rosenfeld, Elan and Kolter, J. Zico},
    pages = {1310--1320},
    publisher = {PMLR},
    isbn = {2640-3498},
    issn = {23318422}
}

@article{Jia2020,
    title = {{Certified robustness of nearest neighbors against data poisoning attacks}},
    year = {2020},
    journal = {arXiv},
    author = {Jia, Jinyuan and Cao, Xiaoyu and Gong, Neil Zhenqiang},
    issn = {23318422},
    arxivId = {2012.03765}
}

@inproceedings{Deng2017,
    title = {{CNN based semantic segmentation for urban traffic scenes using fisheye camera}},
    year = {2017},
    booktitle = {2017 IEEE Intelligent Vehicles Symposium (IV)},
    author = {Deng, Liuyuan and Yang, Ming and Qian, Yeqiang and Wang, Chunxiang and Wang, Bing},
    pages = {231--236},
    publisher = {IEEE},
    isbn = {1509048049}
}

@inproceedings{Checkoway2011c,
    title = {{Comprehensive experimental analyses of automotive attack surfaces}},
    year = {2011},
    booktitle = {Proceedings of the 20th USENIX Security Symposium},
    author = {Checkoway, Stephen and McCoy, Damon and Kantor, Brian and Anderson, Danny and Shacham, Hovav and Savage, Stefan and Koscher, Karl and Czeskis, Alexei and Roesner, Franziska and Kohno, Tadayoshi},
    pages = {77--92},
    volume = {4},
    publisher = {San Francisco},
    isbn = {9781931971874}
}

@article{TURING1950,
    title = {{Computing machinery and}},
    year = {1940},
    journal = {Nature},
    author = {Turing, Alan M. A.M.},
    number = {3678},
    pages = {662--662},
    volume = {145},
    url = {http://mind.oxfordjournals.org/cgi/doi/10.1093/mind/LIX.236.433%0Ahttps://academic.oup.com/mind/article-lookup/doi/10.1093/mind/LIX.236.433%0Ahttp://www.nature.com/articles/145662c0},
    isbn = {9781402085819},
    issn = {0028-0836},
    pmid = {18684640},
    arxivId = {10.2307/2251299}
}

@article{Bozkurt2019b,
    title = {{Control synthesis from linear temporal logic specifications using model-free reinforcement learning}},
    year = {2019},
    journal = {arXiv},
    author = {Bozkurt, Alper Kamil and Wang, Yu and Zavlanos, Michael and Pajic, Miroslav},
    issn = {23318422}
}

@book{Nise2007,
    title = {{Control Systems Engineering}},
    year = {1961},
    booktitle = {or},
    author = {O'Donnell, P. J. and Seifort, William W. and Steeg, Carl W.},
    number = {2},
    pages = {124},
    volume = {12},
    publisher = {John Wiley {\&} Sons},
    isbn = {8126510978},
    doi = {10.2307/3007422},
    issn = {14732858}
}

@book{Boyd2004,
    title = {{Convex optimization}},
    year = {2004},
    author = {Boyd, Stephen and Boyd, Stephen P and Vandenberghe, Lieven},
    publisher = {Cambridge university press},
    isbn = {0521833787}
}

@article{DeSa2017a,
    title = {{Covert Attacks in Cyber-Physical Control Systems}},
    year = {2017},
    journal = {IEEE Transactions on Industrial Informatics},
    author = {De S{\'{a}}, Alan Oliveira and Carmo, Luiz F.Rust Da Costa and Machado, Raphael C.S.},
    number = {4},
    pages = {1641--1651},
    volume = {13},
    publisher = {IEEE},
    doi = {10.1109/TII.2017.2676005},
    issn = {15513203},
    arxivId = {1609.09537},
    keywords = {Cyber-physical systems, networked control systems (NCSs), security}
}

@inproceedings{Teixeira2010a,
    title = {{Cyber security analysis of state estimators in electric power systems}},
    year = {2010},
    booktitle = {Proceedings of the IEEE Conference on Decision and Control},
    author = {Teixeira, André and Amin, Saurabh and Sandberg, Henrik and Johansson, Karl H. and Sastry, Shankar S.},
    pages = {5991--5998},
    publisher = {IEEE},
    isbn = {9781424477456},
    doi = {10.1109/CDC.2010.5717318},
    issn = {01912216}
}

@inproceedings{Pasqualetti2011a,
    title = {{Cyber-physical attacks in power networks: Models, fundamental limitations and monitor design}},
    year = {2011},
    booktitle = {Proceedings of the IEEE Conference on Decision and Control},
    author = {Pasqualetti, Fabio and Dorfler, Florian and Bullo, Francesco},
    pages = {2195--2201},
    publisher = {IEEE},
    isbn = {9781612848006},
    doi = {10.1109/CDC.2011.6160641},
    issn = {01912216},
    arxivId = {1103.2795}
}

@article{Chen2017b,
    title = {{Cyber-Physical Attacks with Control Objectives}},
    year = {2018},
    journal = {IEEE Transactions on Automatic Control},
    author = {Chen, Yuan and Kar, Soummya and Moura, Jose M.F.},
    number = {5},
    pages = {1418--1425},
    volume = {63},
    publisher = {IEEE},
    doi = {10.1109/TAC.2017.2741778},
    issn = {00189286},
    arxivId = {1607.05927},
    keywords = {Attack detection, cyber-physical systems (CPSs), optimal control, security}
}

@article{Mo2011a,
    title = {{Cyber-physical security of a smart grid infrastructure}},
    year = {2012},
    journal = {Proceedings of the IEEE},
    author = {Mo, Yilin and Kim, Tiffany Hyun Jin and Brancik, Kenneth and Dickinson, Dona and Lee, Heejo and Perrig, Adrian and Sinopoli, Bruno},
    number = {1},
    pages = {195--209},
    volume = {100},
    publisher = {IEEE},
    doi = {10.1109/JPROC.2011.2161428},
    issn = {00189219},
    keywords = {Cyber-physical systems, security, smart grids}
}

@article{Bai2017c,
    title = {{Data-injection attacks in stochastic control systems: Detectability and performance tradeoffs *}},
    year = {2017},
    journal = {arXiv},
    author = {Bai, Cheng Zong and Pasqualetti, Fabio and Gupta, Vijay},
    pages = {251--260},
    volume = {82},
    publisher = {Elsevier},
    issn = {23318422},
    keywords = {Cyberphysical system security, Networked control systems, Stochastic systems}
}

@article{Brendel2017,
    title = {{Decision-based adversarial attacks: Reliable attacks against black-box machine learning models}},
    year = {2017},
    journal = {arXiv},
    author = {Brendel, Wieland and Rauber, Jonas and Bethge, Matthias},
    issn = {23318422},
    arxivId = {1712.04248}
}

@inproceedings{Liang2018a,
    title = {{Deep Continuous Fusion for Multi-sensor 3D Object Detection}},
    year = {2018},
    booktitle = {Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
    author = {Liang, Ming and Yang, Bin and Wang, Shenlong and Urtasun, Raquel},
    pages = {663--678},
    volume = {11220 LNCS},
    isbn = {9783030012694},
    doi = {10.1007/978-3-030-01270-0{\_}39},
    issn = {16113349},
    arxivId = {2012.10992},
    keywords = {3D object detection, Autonomous driving, Multi-sensor fusion}
}

@inproceedings{Abadi2016,
    title = {{Deep learning with differential privacy}},
    year = {2016},
    booktitle = {Proceedings of the 2016 ACM SIGSAC conference on computer and communications security},
    author = {Abadi, Martin and Chu, Andy and Goodfellow, Ian and McMahan, H Brendan and Mironov, Ilya and Talwar, Kunal and Zhang, Li},
    pages = {308--318}
}

@inproceedings{Hitaj2017,
    title = {{Deep models under the GAN: information leakage from collaborative deep learning}},
    year = {2017},
    booktitle = {Proceedings of the 2017 ACM SIGSAC Conference on Computer and Communications Security},
    author = {Hitaj, Briland and Ateniese, Giuseppe and Perez-Cruz, Fernando},
    pages = {603--618}
}

@inproceedings{Nguyen2015b,
    title = {{Deep neural networks are easily fooled: High confidence predictions for unrecognizable images}},
    year = {2015},
    booktitle = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
    author = {Nguyen, Anh and Yosinski, Jason and Clune, Jeff},
    pages = {427--436},
    volume = {07-12-June},
    isbn = {9781467369640},
    doi = {10.1109/CVPR.2015.7298640},
    issn = {10636919},
    arxivId = {1412.1897}
}

@inproceedings{Moosavi-Dezfooli2016a,
    title = {{DeepFool: A Simple and Accurate Method to Fool Deep Neural Networks}},
    year = {2016},
    booktitle = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
    author = {Moosavi-Dezfooli, Seyed Mohsen and Fawzi, Alhussein and Frossard, Pascal},
    pages = {2574--2582},
    volume = {2016-Decem},
    isbn = {9781467388504},
    doi = {10.1109/CVPR.2016.282},
    issn = {10636919},
    arxivId = {1511.04599}
}

@article{Samangouei2018b,
    title = {{Defense-gan: Protecting classifiers against adversarial attacks using generative models}},
    year = {2018},
    journal = {arXiv},
    author = {Samangouei, Pouya and Kabkab, Maya and Chellappa, Rama},
    issn = {23318422},
    arxivId = {1805.06605}
}

@inproceedings{Zhang2019b,
    title = {{Defense-PointNet: Protecting PointNet against adversarial attacks}},
    year = {2020},
    booktitle = {arXiv},
    author = {Zhang, Yu and Liang, Gongbo and Salem, Tawfiq and Jacobs, Nathan},
    pages = {5654--5660},
    publisher = {IEEE},
    isbn = {1728108586},
    issn = {23318422},
    keywords = {Adversarial attack, Defensive network, Point cloud, Pointnet}
}

@article{Pajic2017a,
    title = {{Design and Implementation of Attack-Resilient Cyberphysical Systems: With a Focus on Attack-Resilient State Estimators}},
    year = {2017},
    journal = {IEEE Control Systems},
    author = {Pajic, Miroslav and Weimer, James and Bezzo, Nicola and Sokolsky, Oleg and Pappas, George J. and Lee, Insup},
    number = {2},
    pages = {66--81},
    volume = {37},
    publisher = {IEEE},
    doi = {10.1109/MCS.2016.2643239},
    issn = {1066033X}
}

@inproceedings{Hoehn2016a,
    title = {{Detection of replay attacks in cyber-physical systems}},
    year = {2016},
    booktitle = {Proceedings of the American Control Conference},
    author = {Hoehn, Andreas and Zhang, Ping},
    pages = {290--295},
    volume = {2016-July},
    publisher = {IEEE},
    isbn = {9781467386821},
    doi = {10.1109/ACC.2016.7524930},
    issn = {07431619}
}

@inproceedings{Papernot2016,
    title = {{Distillation as a defense to adversarial perturbations against deep neural networks}},
    year = {2016},
    booktitle = {2016 IEEE symposium on security and privacy (SP)},
    author = {Papernot, Nicolas and McDaniel, Patrick and Wu, Xi and Jha, Somesh and Swami, Ananthram},
    pages = {582--597},
    publisher = {IEEE},
    isbn = {1509008241}
}

@article{Sundaram2010a,
    title = {{Distributed function calculation via linear iterative strategies in the presence of malicious agents}},
    year = {2011},
    journal = {IEEE Transactions on Automatic Control},
    author = {Sundaram, Shreyas and Hadjicostis, Christoforos N.},
    number = {7},
    pages = {1495--1508},
    volume = {56},
    publisher = {IEEE},
    doi = {10.1109/TAC.2010.2088690},
    issn = {00189286},
    keywords = {Distributed consensus, distributed function calculation, fault-tolerant consensus, multi-agent systems, networked control, observability theory, structured systems, wireless broadcast model}
}

@article{Liu2018,
    title = {{Dpatch: An adversarial patch attack on object detectors}},
    year = {2018},
    journal = {arXiv},
    author = {Liu, Xin and Yang, Huanrui and Liu, Ziwei and Song, Linghao and Li, Hai and Chen, Yiran},
    issn = {23318422},
    arxivId = {1806.02299}
}

@article{Shen2020c,
    title = {{Drift with Devil: Security of Multi-Sensor Fusion based Localization in High-Level Autonomous Driving under GPS Spoofing (Extended Version)}},
    year = {2020},
    journal = {arXiv},
    author = {Shen, Junjie and Won, Jun Yeon and Chen, Zeyuan and Chen, Qi Alfred},
    issn = {23318422}
}

@inproceedings{Zhou2019b,
    title = {{DUP-net: Denoiser and upsampler network for 3D adversarial point clouds defense}},
    year = {2019},
    booktitle = {Proceedings of the IEEE International Conference on Computer Vision},
    author = {Zhou, Hang and Chen, Kejiang and Zhang, Weiming and Fang, Han and Zhou, Wenbo and Yu, Nenghai},
    pages = {1961--1970},
    volume = {2019-Octob},
    isbn = {9781728148038},
    doi = {10.1109/ICCV.2019.00205},
    issn = {15505499},
    arxivId = {1812.11017}
}

@inproceedings{Ma2020b,
    title = {{Efficient Joint Gradient Based Attack Against SOR Defense for 3D Point Cloud Classification}},
    year = {2020},
    booktitle = {Proceedings of the 28th ACM International Conference on Multimedia},
    author = {Ma, Chengcheng and Meng, Weiliang and Wu, Baoyuan and Xu, Shibiao and Zhang, Xiaopeng},
    pages = {1819--1827},
    doi = {10.1145/3394171.3413875}
}

@inproceedings{Kohli2019,
    title = {{Enabling pedestrian safety using computer vision techniques: A case study of the 2018 uber inc. self-driving car crash}},
    year = {2019},
    booktitle = {Future of Information and Communication Conference},
    author = {Kohli, Puneet and Chadha, Anjali},
    pages = {261--279},
    publisher = {Springer}
}

@inproceedings{Codevilla2018,
    title = {{End-to-End Driving Via Conditional Imitation Learning}},
    year = {2018},
    booktitle = {Proceedings - IEEE International Conference on Robotics and Automation},
    author = {Codevilla, Felipe and Miiller, Matthias and Lopez, Antonio and Koltun, Vladlen and Dosovitskiy, Alexey},
    pages = {4693--4700},
    url = {https://github.com/carla-simulator/},
    isbn = {9781538630815},
    doi = {10.1109/ICRA.2018.8460487},
    issn = {10504729},
    arxivId = {1710.02410}
}

@article{Shoukry2015b,
    title = {{Event-triggered state observers for sparse sensor noise/attacks}},
    year = {2016},
    journal = {IEEE Transactions on Automatic Control},
    author = {Shoukry, Yasser and Tabuada, Paulo},
    number = {8},
    pages = {2079--2091},
    volume = {61},
    publisher = {IEEE},
    doi = {10.1109/TAC.2015.2492159},
    issn = {00189286},
    arxivId = {1309.3511},
    keywords = {Event-triggered observers, secure cyber-physical systems, secure state reconstruction, sensor attacks}
}

@inproceedings{Koscher2010b,
    title = {{Experimental security analysis of a modern automobile}},
    year = {2010},
    booktitle = {Proceedings - IEEE Symposium on Security and Privacy},
    author = {Koscher, Karl and Czeskis, Alexei and Roesner, Franziska and Patel, Shwetak and Kohno, Tadayoshi and Checkoway, Stephen and McCoy, Damon and Kantor, Brian and Anderson, Danny and Snach{\'{a}}m, Hovav and Savage, Stefan},
    pages = {447--462},
    publisher = {IEEE},
    isbn = {9780769540351},
    doi = {10.1109/SP.2010.34},
    issn = {10816011},
    keywords = {Automobiles, Communication standards, Communication system security, Computer security, Data buses}
}

@article{Puiutta2020b,
    title = {{Explainable Reinforcement Learning: A Survey}},
    year = {2020},
    journal = {arXiv},
    author = {Puiutta, Erika and Veith, Eric M.S.P.},
    issn = {23318422},
    keywords = {Machine Learning {\textperiodcentered} Explainable {\textperiodcentered} Reinforcement Lea}
}

@article{Goodfellow2014a,
    title = {{Explaining and harnessing adversarial examples}},
    year = {2015},
    journal = {3rd International Conference on Learning Representations, ICLR 2015 - Conference Track Proceedings},
    author = {Goodfellow, Ian J. and Shlens, Jonathon and Szegedy, Christian},
    arxivId = {1412.6572}
}

@article{Tu2021b,
    title = {{Exploring Adversarial Robustness of Multi-Sensor Perception Systems in Self Driving}},
    year = {2021},
    journal = {arXiv preprint arXiv:2101.06784},
    author = {Tu, James and Li, Huichen and Yan, Xinchen and Ren, Mengye and Chen, Yun and Liang, Ming and Bitar, Eilyan and Yumer, Ersin and Urtasun, Raquel},
    url = {http://arxiv.org/abs/2101.06784},
    arxivId = {2101.06784}
}

@inproceedings{Chen2018b,
    title = {{Exposing Congestion Attack on Emerging Connected Vehicle based Traffic Signal Control}},
    year = {2018},
    booktitle = {NDSS},
    author = {Chen, Qi Alfred and Yin, Yucheng and Feng, Yiheng and Mao, Z. Morley and Liu, Henry X.},
    doi = {10.14722/ndss.2018.23222}
}

@inproceedings{Liu2019c,
    title = {{Extending adversarial attacks and defenses to deep 3D point cloud classifiers}},
    year = {2019},
    booktitle = {arXiv},
    author = {Liu, Daniel and Yu, Ronald and Su, Hao},
    pages = {2279--2283},
    publisher = {IEEE},
    isbn = {1538662493},
    issn = {23318422}
}

@inproceedings{Mo2010a,
    title = {{False data injection attacks in healthcare}},
    year = {2018},
    booktitle = {Communications in Computer and Information Science},
    author = {Ahmed, Mohiuddin and Barkat Ullah, Abu S.S.M.},
    pages = {192--202},
    volume = {845},
    isbn = {9789811302916},
    doi = {10.1007/978-981-13-0292-3{\_}12},
    issn = {18650929},
    keywords = {FDIA, Healthcare, Smart grid}
}

@inproceedings{Girshick2015,
    title = {{Fast r-cnn}},
    year = {2015},
    booktitle = {Proceedings of the IEEE international conference on computer vision},
    author = {Girshick, Ross},
    pages = {1440--1448}
}

@article{Balta2018b,
    title = {{Fast Statistical Outlier Removal Based Method for Large 3D Point Clouds of Outdoor Environments}},
    year = {2018},
    journal = {IFAC-PapersOnLine},
    author = {Balta, Haris and Velagic, Jasmin and Bosschaerts, Walter and De Cubber, Geert and Siciliano, Bruno},
    number = {22},
    pages = {348--353},
    volume = {51},
    publisher = {Elsevier},
    doi = {10.1016/j.ifacol.2018.11.566},
    issn = {24058963},
    keywords = {3D point cloud, FCSOR, Unmanned ground vehicle, large-scale environment, outlier removal}
}

@article{Ren2015,
    title = {{Faster r-cnn: Towards real-time object detection with region proposal networks}},
    year = {2015},
    journal = {arXiv preprint arXiv:1506.01497},
    author = {Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian}
}

@inproceedings{Lin2017,
    title = {{Feature pyramid networks for object detection}},
    year = {2017},
    booktitle = {Proceedings of the IEEE conference on computer vision and pattern recognition},
    author = {Lin, Tsung-Yi and Doll{\'{a}}r, Piotr and Girshick, Ross and He, Kaiming and Hariharan, Bharath and Belongie, Serge},
    pages = {2117--2125}
}

@book{Astrom2010,
    title = {{Feedback systems: An introduction for scientists and engineers}},
    year = {2010},
    booktitle = {Feedback Systems: An Introduction for Scientists and Engineers},
    author = {Johan {\AA}str{\"{o}}m, Karl and Murray, Richard M.},
    publisher = {Princeton university press},
    isbn = {0691135762},
    doi = {10.5860/choice.46-2107},
    issn = {0009-4978}
}

@inproceedings{Jia2020a,
    title = {{Fooling Detection Alone is Not Enough: First Adversarial Attack against Multiple Object Tracking}},
    year = {2020},
    booktitle = {International Conference on Learning Representations (ICLR)},
    author = {Jia, Yunhan and Lu, Yantao and Shen, Junjie and Chen, Qi A and Zhong, Zhenyu and Wei, Tao}
}

@article{Wang2019c,
    title = {{Frustum ConvNet: Sliding Frustums to Aggregate Local Point-Wise Features for Amodal}},
    year = {2019},
    journal = {IEEE International Conference on Intelligent Robots and Systems},
    author = {Wang, Zhixin and Jia, Kui},
    pages = {1742--1749},
    isbn = {9781728140049},
    doi = {10.1109/IROS40897.2019.8968513},
    issn = {21530866}
}

@inproceedings{Qi2018b,
    title = {{Frustum PointNets for 3D Object Detection from RGB-D Data}},
    year = {2018},
    booktitle = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
    author = {Qi, Charles R. and Liu, Wei and Wu, Chenxia and Su, Hao and Guibas, Leonidas J.},
    pages = {918--927},
    isbn = {9781538664209},
    doi = {10.1109/CVPR.2018.00102},
    issn = {10636919},
    arxivId = {1711.08488}
}

@article{Manshaei2013a,
    title = {{Game-based analysis of the network attack-defense interaction}},
    year = {2014},
    journal = {Lecture Notes in Engineering and Computer Science},
    author = {Alese, Boniface K. and Ibidunmoye, Emmanuel O. and Haruna, D. I. and Thompson, Aderonke F. and Otasowie, Iyare},
    number = {3},
    pages = {481--487},
    volume = {1},
    publisher = {ACM New York, NY, USA},
    isbn = {9789881925275},
    issn = {20780958},
    keywords = {Attackers, Defenders, Deterministic games, Game theory, Security games, Stochastic games, Strategies}
}

@inproceedings{Xiang2019c,
    title = {{Generating 3d adversarial point clouds}},
    year = {2018},
    booktitle = {arXiv},
    author = {Xiang, Chong and Qi, Charles R. and Li, Bo},
    pages = {9136--9144},
    issn = {23318422}
}

@article{Hu2017b,
    title = {{Generating adversarial malware examples for black-box attacks based on gan}},
    year = {2017},
    journal = {arXiv},
    author = {Hu, Weiwei and Tan, Ying},
    issn = {23318422},
    arxivId = {1702.05983}
}

@article{Goodfellow2014,
    title = {{Generative adversarial networks}},
    year = {2014},
    journal = {arXiv preprint arXiv:1406.2661},
    author = {Goodfellow, Ian J and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua}
}

@article{Lang2020a,
    title = {{Geometric adversarial attacks and defenses on 3D point clouds}},
    year = {2020},
    journal = {arXiv},
    author = {Lang, Itai and Kotlicki, Uriel and Avidan, Shai},
    issn = {23318422},
    arxivId = {2012.05657}
}

@article{Wen2019c,
    title = {{Geometry-aware generation of adversarial and cooperative point clouds}},
    year = {2019},
    journal = {arXiv},
    author = {Wen, Yuxin and Lin, Jiehong and Chen, Ke and Jia, Kui},
    issn = {23318422}
}

@article{Doyle1978,
    title = {{Guaranteed Margins for LQG Regulators}},
    year = {1978},
    journal = {IEEE Transactions on Automatic Control},
    author = {Doyle, John C.},
    number = {4},
    pages = {756--757},
    volume = {23},
    publisher = {IEEE},
    doi = {10.1109/TAC.1978.1101812},
    issn = {15582523}
}

@inproceedings{Chen2020b,
    title = {{Hopskipjumpattack: A query-efficient decision-based attack}},
    year = {2020},
    booktitle = {2020 ieee symposium on security and privacy (sp)},
    author = {Chen, Jianbo and Jordan, Michael I and Wainwright, Martin J},
    pages = {1277--1294},
    publisher = {IEEE},
    isbn = {1728134978}
}

@article{Cisse2017b,
    title = {{Houdini: Fooling deep structured prediction models}},
    year = {2017},
    journal = {arXiv},
    author = {Cisse, Moustapha and Adi, Yossi and Neverova, Natalia and Keshet, Joseph},
    issn = {23318422},
    arxivId = {1707.05373}
}

@article{Mnih2015b,
    title = {{Human-level control through deep reinforcement learning}},
    year = {2015},
    journal = {Nature},
    author = {Mnih, Volodymyr and Kavukcuoglu, Koray and Silver, David and Rusu, Andrei A. and Veness, Joel and Bellemare, Marc G. and Graves, Alex and Riedmiller, Martin and Fidjeland, Andreas K. and Ostrovski, Georg and Petersen, Stig and Beattie, Charles and Sadik, Amir and Antonoglou, Ioannis and King, Helen and Kumaran, Dharshan and Wierstra, Daan and Legg, Shane and Hassabis, Demis},
    number = {7540},
    pages = {529--533},
    volume = {518},
    publisher = {Nature Publishing Group},
    doi = {10.1038/nature14236},
    issn = {14764687},
    pmid = {25719670}
}

@inproceedings{Shin2017d,
    title = {{Illusion and dazzle: Adversarial optical channel exploits against lidars for automotive applications}},
    year = {2017},
    booktitle = {Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
    author = {Shin, Hocheol and Kim, Dohyun and Kwon, Yujin and Kim, Yongdae},
    pages = {445--467},
    volume = {10529 LNCS},
    publisher = {Springer},
    isbn = {9783319667867},
    doi = {10.1007/978-3-319-66787-4{\_}22},
    issn = {16113349},
    keywords = {Attack, Autonomous car, Lidar, Saturating, Sensor, Spoofing}
}

@article{Weber2017b,
    title = {{Imagination-augmented agents for deep reinforcement learning}},
    year = {2017},
    journal = {arXiv},
    author = {Weber, Theóphane and Racani{\`{e}}re, Sébastien and Reichert, David P. and Buesing, Lars and Guez, Arthur and Rezende, Danilo and Badia, Adria Puigdomènech and Vinyals, Oriol and Heess, Nicolas and Li, Yujia and Pascanu, Razvan and Battaglia, Peter and Hassabis, Demis and Silver, David and Wierstra, Daan},
    issn = {23318422}
}

@inproceedings{Worner2016c,
    title = {{Integrity for autonomous driving: A survey}},
    year = {2016},
    booktitle = {Proceedings of the IEEE/ION Position, Location and Navigation Symposium, PLANS 2016},
    author = {Worner, M. and Schuster, F. and Dolitzscher, F. and Keller, C. G. and Haueis, M. and Dietmayer, K.},
    pages = {666--671},
    publisher = {IEEE},
    isbn = {9781509020423},
    doi = {10.1109/PLANS.2016.7479759}
}

@inproceedings{Ghorbani2019,
    title = {{Interpretation of neural networks is fragile}},
    year = {2019},
    booktitle = {Proceedings of the AAAI Conference on Artificial Intelligence},
    author = {Ghorbani, Amirata and Abid, Abubakar and Zou, James},
    number = {01},
    pages = {3681--3688},
    volume = {33},
    isbn = {2374-3468}
}

@article{Szegedy2013b,
    title = {{Intriguing properties of neural networks}},
    year = {2014},
    journal = {2nd International Conference on Learning Representations, ICLR 2014 - Conference Track Proceedings},
    author = {Szegedy, Christian and Zaremba, Wojciech and Sutskever, Ilya and Bruna, Joan and Erhan, Dumitru and Goodfellow, Ian and Fergus, Rob},
    arxivId = {1312.6199}
}

@article{Yu2020,
    title = {{Investigating vulnerability to adversarial examples on multimodal data fusion in deep learning}},
    year = {2020},
    journal = {arXiv},
    author = {Yu, Youngjoon and Lee, Hong Joo and Kim, Byeong Cheon and Kim, Jung Uk and Ro, Yong Man},
    issn = {23318422},
    arxivId = {2005.10987}
}

@inproceedings{Ku2018,
    title = {{Joint 3D Proposal Generation and Object Detection from View Aggregation}},
    year = {2018},
    booktitle = {IEEE International Conference on Intelligent Robots and Systems},
    author = {Ku, Jason and Mozifian, Melissa and Lee, Jungwook and Harakeh, Ali and Waslander, Steven L.},
    pages = {5750--5757},
    publisher = {IEEE},
    isbn = {9781538680940},
    doi = {10.1109/IROS.2018.8594049},
    issn = {21530866},
    arxivId = {1712.02294}
}

@inproceedings{Iandola2017,
    title = {{Keynote: small neural nets are beautiful: enabling embedded systems with small deep-neural-network architectures}},
    year = {2017},
    booktitle = {2017 International Conference on Hardware/Software Codesign and System Synthesis (CODES+ ISSS)},
    author = {Iandola, Forrest and Keutzer, Kurt},
    pages = {1--10},
    publisher = {IEEE},
    isbn = {1450351859}
}

@inproceedings{Shrikumar2017,
    title = {{Learning important features through propagating activation differences}},
    year = {2017},
    booktitle = {International Conference on Machine Learning},
    author = {Shrikumar, Avanti and Greenside, Peyton and Kundaje, Anshul},
    pages = {3145--3153},
    publisher = {PMLR},
    isbn = {2640-3498}
}

@article{Khojasteh2020b,
    title = {{Learning-based attacks in cyber-physical systems}},
    year = {2021},
    journal = {IEEE Transactions on Control of Network Systems},
    author = {Khojasteh, Mohammad Javad and Khina, Anatoly and Franceschetti, Massimo and Javidi, Tara},
    number = {1},
    pages = {437--449},
    volume = {8},
    publisher = {IEEE},
    doi = {10.1109/TCNS.2020.3028035},
    issn = {23255870},
    keywords = {Cyber-physical system security, learning for dynamics and control, man-in-the-middle attack, physical layer authentication, secure control, system identification}
}

@inproceedings{Zhou2020b,
    title = {{LG-GAN: Label guided adversarial network for flexible targeted attack of point cloud-based deep networks}},
    year = {2020},
    booktitle = {arXiv},
    author = {Zhou, Hang and Chen, Dongdong and Liao, Jing and Chen, Kejiang and Dong, Xiaoyi and Liu, Kunlin and Zhang, Weiming and Hua, Gang and Yu, Nenghai},
    pages = {10356--10365},
    issn = {23318422}
}

@article{Changalvala2019c,
    title = {{LiDAR Data Integrity Verification for Autonomous Vehicle Using 3D Data Hiding}},
    year = {2019},
    journal = {2019 IEEE Symposium Series on Computational Intelligence, SSCI 2019},
    author = {Changalvala, Raghu and Malik, Hafiz},
    pages = {1219--1225},
    volume = {7},
    publisher = {IEEE},
    isbn = {9781728124858},
    doi = {10.1109/SSCI44817.2019.9002737},
    issn = {15502252},
    keywords = {ADAS, Autonomous vehicle, LiDAR point cloud, data hiding, quantization index modulation (QIM), sensor data integrity}
}

@article{Hecht2018,
    title = {{Lidar for self-driving cars}},
    year = {2018},
    journal = {Optics and Photonics News},
    author = {Hecht, Jeff},
    number = {1},
    pages = {26--33},
    volume = {29},
    publisher = {Optical Society of America},
    issn = {1541-3721}
}

@book{Rugh1996a,
    title = {{Linear system theory}},
    year = {1994},
    booktitle = {Automatica},
    author = {Kennedy, R.A.},
    number = {11},
    pages = {1811--1813},
    volume = {30},
    publisher = {Prentice-Hall, Inc.},
    isbn = {0134412052},
    doi = {10.1016/0005-1098(94)90090-6},
    issn = {00051098}
}

@inproceedings{Fang2020d,
    title = {{Local model poisoning attacks to byzantine-robust federated learning}},
    year = {2019},
    booktitle = {arXiv},
    author = {Fang, Minghong and Cao, Xiaoyu and Jia, Jinyuan and Gong, Neil Zhenqiang},
    pages = {1605--1622},
    isbn = {1939133173},
    issn = {23318422}
}

@article{Mitchell1999,
    title = {{Machine learning and data mining}},
    year = {2007},
    journal = {Machine Learning and Data Mining},
    author = {Kononenko, Igor and Kukar, Matjaž},
    number = {11},
    pages = {30--36},
    volume = {42},
    publisher = {ACM New York, NY, USA},
    isbn = {9781904275213},
    doi = {10.1533/9780857099440},
    issn = {0001-0782}
}

@inproceedings{Shokri2017,
    title = {{Membership Inference Attacks Against Machine Learning Models}},
    year = {2017},
    booktitle = {Proceedings - IEEE Symposium on Security and Privacy},
    author = {Shokri, Reza and Stronati, Marco and Song, Congzheng and Shmatikov, Vitaly},
    pages = {3--18},
    publisher = {IEEE},
    isbn = {9781509055326},
    doi = {10.1109/SP.2017.41},
    issn = {10816011},
    arxivId = {1610.05820}
}

@inproceedings{Xiao2018,
    title = {{MeshAdv: Adversarial Meshes for Visual Recognition}},
    year = {2018},
    booktitle = {arXiv},
    author = {Xiao, Chaowei and Yang, Dawei and Deng, Jia and Liu, Mingyan and Li, Bo},
    pages = {6898--6907},
    issn = {23318422}
}

@book{Ogata2002,
    title = {{Modern control engineering}},
    year = {2017},
    booktitle = {Modern Control Engineering},
    author = {Paraskevopoulos, P. N.},
    pages = {1--736},
    volume = {4},
    publisher = {Prentice hall India},
    isbn = {9781482277449},
    doi = {10.1201/9781315214573}
}

@inproceedings{Obst2014b,
    title = {{Multi-sensor data fusion for checking plausibility of V2V communications by vision-based multiple-object tracking}},
    year = {2015},
    booktitle = {IEEE Vehicular Networking Conference, VNC},
    author = {Obst, Marcus and Hobert, Laurens and Reisdorf, Pierre},
    number = {January},
    pages = {143--150},
    volume = {2015-Janua},
    publisher = {IEEE},
    isbn = {9781479976607},
    doi = {10.1109/VNC.2014.7013333},
    issn = {21579865}
}

@inproceedings{Liang2019,
    title = {{Multi-task multi-sensor fusion for 3D object detection}},
    year = {2019},
    booktitle = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
    author = {Liang, Ming and Yang, Bin and Chen, Yun and Hu, Rui and Urtasun, Raquel},
    pages = {7337--7345},
    volume = {2019-June},
    isbn = {9781728132938},
    doi = {10.1109/CVPR.2019.00752},
    issn = {10636919},
    arxivId = {2012.12397},
    keywords = {3D from Multiview and Sensors, Categorization, Deep Learning, Recognition: Detection, Representation Learning, Retrieval, Robotics + Driving}
}

@inproceedings{Chen2017c,
    title = {{Multi-view 3D object detection network for autonomous driving}},
    year = {2017},
    booktitle = {Proceedings - 30th IEEE Conference on Computer Vision and Pattern Recognition, CVPR 2017},
    author = {Chen, Xiaozhi and Ma, Huimin and Wan, Ji and Li, Bo and Xia, Tian},
    pages = {6526--6534},
    volume = {2017-Janua},
    isbn = {9781538604571},
    doi = {10.1109/CVPR.2017.691},
    arxivId = {1611.07759}
}

@article{Blackman1986,
    title = {{Multiple-target tracking with radar applications}},
    year = {1986},
    journal = {Dedham},
    author = {Blackman, Samuel S}
}

@article{Doyle1981,
    title = {{Multivariable Feedback Design: Concepts for a Classical/Modern Synthesis}},
    year = {1981},
    journal = {IEEE Transactions on Automatic Control},
    author = {Doyle, John C. and Stein, Gunter},
    number = {1},
    pages = {4--16},
    volume = {26},
    publisher = {IEEE},
    doi = {10.1109/TAC.1981.1102555},
    issn = {15582523}
}

@inproceedings{Sindagi2019,
    title = {{Mvx-net: Multimodal voxelnet for 3d object detection}},
    year = {2019},
    booktitle = {2019 International Conference on Robotics and Automation (ICRA)},
    author = {Sindagi, Vishwanath A and Zhou, Yin and Tuzel, Oncel},
    pages = {7276--7282},
    publisher = {IEEE},
    isbn = {153866027X}
}

@inproceedings{Wang2019a,
    title = {{Neural cleanse: Identifying and mitigating backdoor attacks in neural networks}},
    year = {2019},
    booktitle = {Proceedings - IEEE Symposium on Security and Privacy},
    author = {Wang, Bolun and Yao, Yuanshun and Shan, Shawn and Li, Huiying and Viswanath, Bimal and Zheng, Haitao and Zhao, Ben Y.},
    pages = {707--723},
    volume = {2019-May},
    publisher = {IEEE},
    isbn = {9781538666609},
    doi = {10.1109/SP.2019.00031},
    issn = {10816011},
    keywords = {Backdoor-Attack, Deep-Learning, Security}
}

@inproceedings{Shoukry2013a,
    title = {{Non-invasive spoofing attacks for anti-lock braking systems}},
    year = {2013},
    booktitle = {Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
    author = {Shoukry, Yasser and Martin, Paul and Tabuada, Paulo and Srivastava, Mani},
    pages = {55--72},
    volume = {8086 LNCS},
    publisher = {Springer},
    isbn = {9783642403484},
    doi = {10.1007/978-3-642-40349-1{\_}4},
    issn = {16113349},
    keywords = {Automotive embedded systems, Cyber-physical security, Magnetic sensors, Non-invasive sensor attacks}
}

@article{Zhao2020,
    title = {{Nudge Attacks on Point-Cloud DNNs}},
    year = {2020},
    journal = {arXiv preprint arXiv:2011.11637},
    author = {Zhao, Yiren and Shumailov, Ilia and Mullins, Robert and Anderson, Ross}
}

@book{Nocedal2006,
    title = {{Numerical optimization}},
    year = {2006},
    author = {Nocedal, Jorge and Wright, Stephen},
    publisher = {Springer Science {\&} Business Media},
    isbn = {0387400656}
}

@inproceedings{Caesar2020,
    title = {{nuscenes: A multimodal dataset for autonomous driving}},
    year = {2020},
    booktitle = {Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
    author = {Caesar, Holger and Bankiti, Varun and Lang, Alex H and Vora, Sourabh and Liong, Venice Erin and Xu, Qiang and Krishnan, Anush and Pan, Yu and Baldan, Giancarlo and Beijbom, Oscar},
    pages = {11621--11631}
}

@inproceedings{Athalye2018b,
    title = {{Obfuscated gradients give a false sense of security: Circumventing defenses to adversarial examples}},
    year = {2018},
    booktitle = {International Conference on Machine Learning},
    author = {Athalye, Anish and Carlini, Nicholas and Wagner, David},
    pages = {274--283},
    publisher = {PMLR},
    isbn = {2640-3498},
    issn = {23318422}
}

@inproceedings{Athalye2018,
    title = {{Obfuscated gradients give a false sense of security: Circumventing defenses to adversarial examples}},
    year = {2018},
    booktitle = {International Conference on Machine Learning},
    author = {Athalye, Anish and Carlini, Nicholas and Wagner, David},
    pages = {274--283},
    publisher = {PMLR},
    isbn = {2640-3498}
}

@article{Hau2021a,
    title = {{Object Removal Attacks on LiDAR-based 3D Object Detectors}},
    year = {2021},
    journal = {arXiv preprint arXiv:2102.03722},
    author = {Hau, Zhongyuan and Co, Kenneth T and Demetriou, Soteris and Lupu, Emil C}
}

@article{Bai2017b,
    title = {{On kalman filtering with compromised sensors: Attack stealthiness and performance bounds}},
    year = {2017},
    journal = {IEEE Transactions on Automatic Control},
    author = {Bai, Cheng Zong and Gupta, Vijay and Pasqualetti, Fabio},
    number = {12},
    pages = {6641--6648},
    volume = {62},
    publisher = {IEEE},
    doi = {10.1109/TAC.2017.2714903},
    issn = {00189286},
    keywords = {Detection of stealthy malicious attacks, Kullback-Leibler divergence, Security of cyberphysical systems}
}

@article{Sun2020i,
    title = {{On the adversarial robustness of 3D point cloud classification}},
    year = {2020},
    journal = {arXiv},
    author = {Sun, Jiachen and Koenig, Karl and Cao, Yulong and Chen, Qi Alfred and Mao, Z. Morley},
    issn = {23318422},
    arxivId = {2011.11922}
}

@article{Mo2015b,
    title = {{On the Performance Degradation of Cyber-Physical Systems under Stealthy Integrity Attacks}},
    year = {2016},
    journal = {IEEE Transactions on Automatic Control},
    author = {Mo, Yilin and Sinopoli, Bruno},
    number = {9},
    pages = {2618--2624},
    volume = {61},
    publisher = {IEEE},
    doi = {10.1109/TAC.2015.2498708},
    issn = {00189286},
    keywords = {SCADA systems, robustness, security}
}

@inproceedings{Tippenhauer2011a,
    title = {{On the requirements for successful GPS spoofing attacks}},
    year = {2011},
    booktitle = {Proceedings of the ACM Conference on Computer and Communications Security},
    author = {Tippenhauer, Nils Ole and P{\"{o}}pper, Christina and Rasmussen, Kasper B. and {\v{C}}apkun, Srdjan},
    pages = {75--85},
    isbn = {9781450310758},
    doi = {10.1145/2046707.2046719},
    issn = {15437221},
    keywords = {Experimentation, Security}
}

@article{Su2019a,
    title = {{One pixel attack for fooling deep neural networks}},
    year = {2019},
    journal = {IEEE Transactions on Evolutionary Computation},
    author = {Su, Jiawei and Vargas, Danilo Vasconcellos and Sakurai, Kouichi},
    number = {5},
    pages = {828--841},
    volume = {23},
    publisher = {IEEE},
    issn = {1089-778X}
}

@inproceedings{Gupta2010a,
    title = {{Optimal control in the presence of an intelligent jammer with limited actions}},
    year = {2010},
    booktitle = {Proceedings of the IEEE Conference on Decision and Control},
    author = {Gupta, Abhishek and Langbort, Cédric and Ba{\c{s}}ar, Tamer},
    pages = {1096--1101},
    publisher = {IEEE},
    isbn = {9781424477456},
    doi = {10.1109/CDC.2010.5717544},
    issn = {01912216}
}

@article{Guo2016a,
    title = {{Optimal Linear Cyber-Attack on Remote State Estimation}},
    year = {2017},
    journal = {IEEE Transactions on Control of Network Systems},
    author = {Guo, Ziyang and Shi, Dawei and Johansson, Karl Henrik and Shi, Ling},
    number = {1},
    pages = {4--13},
    volume = {4},
    publisher = {IEEE},
    doi = {10.1109/TCNS.2016.2570003},
    issn = {23255870},
    keywords = {Cyber-physical systems, deception attack, remote state estimation, security}
}

@book{Krause2005c,
    title = {{Optimal nonmyopic value of information in graphical models - Efficient algorithms and theoretical limits}},
    year = {2005},
    booktitle = {IJCAI International Joint Conference on Artificial Intelligence},
    author = {Krause, Andreas and Guestrin, Carlos},
    pages = {1339--1345},
    publisher = {Carnegie Mellon University. Center for Automated Learning and Discovery},
    issn = {10450823}
}

@article{Krause2009c,
    title = {{Optimizing sensing: From water to the web}},
    year = {2009},
    journal = {Computer},
    author = {Krause, Andreas and Guestrin, Carlos},
    number = {8},
    pages = {38--45},
    volume = {42},
    publisher = {IEEE},
    doi = {10.1109/MC.2009.265},
    issn = {00189162}
}

@inproceedings{Song2018b,
    title = {{Physical adversarial examples for object detectors}},
    year = {2018},
    booktitle = {arXiv},
    author = {Eykholt, Kevin and Evtimov, Ivan and Fernandes, Earlence and Li, Bo and Rahmati, Amir and Tram{\`{e}}r, Florian and Prakash, Atul and Kohno, Tadayoshi and Song, Dawn},
    issn = {23318422},
    arxivId = {1807.07769}
}

@article{Mo2015c,
    title = {{Physical authentication of control systems: Designing watermarked control inputs to detect counterfeit sensor outputs}},
    year = {2015},
    journal = {IEEE Control Systems},
    author = {Mo, Yilin and Weerakkody, Sean and Sinopoli, Bruno},
    number = {1},
    pages = {93--109},
    volume = {35},
    publisher = {IEEE},
    doi = {10.1109/MCS.2014.2364724},
    issn = {1066033X}
}

@inproceedings{Tu2020,
    title = {{Physically realizable adversarial examples for LiDAR object detection}},
    year = {2020},
    booktitle = {arXiv},
    author = {Tu, James and Ren, Mengye and Manivasagam, Siva and Liang, Ming and Yang, Bin and Du, Richard and Cheng, Frank and Urtasun, Raquel},
    pages = {13716--13725},
    issn = {23318422}
}

@inproceedings{Yang2018a,
    title = {{PIXOR: Real-time 3D Object Detection from Point Clouds}},
    year = {2018},
    booktitle = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
    author = {Yang, Bin and Luo, Wenjie and Urtasun, Raquel},
    pages = {7652--7660},
    isbn = {9781538664209},
    doi = {10.1109/CVPR.2018.00798},
    issn = {10636919},
    arxivId = {1902.06326}
}

@inproceedings{Zheng2018,
    title = {{PointCloud Saliency Maps}},
    year = {2018},
    booktitle = {arXiv},
    author = {Zheng, Tianhang and Chen, Changyou and Yuan, Junsong and Li, Bo and Ren, Kui},
    pages = {1598--1606},
    issn = {23318422}
}

@inproceedings{Qi2017b,
    title = {{PointNet: Deep learning on point sets for 3D classification and segmentation}},
    year = {2017},
    booktitle = {Proceedings - 30th IEEE Conference on Computer Vision and Pattern Recognition, CVPR 2017},
    author = {Qi, Charles R. and Su, Hao and Mo, Kaichun and Guibas, Leonidas J.},
    pages = {77--85},
    volume = {2017-Janua},
    isbn = {9781538604571},
    doi = {10.1109/CVPR.2017.16},
    arxivId = {1612.00593}
}

@inproceedings{Vora2020,
    title = {{Pointpainting: Sequential fusion for 3d object detection}},
    year = {2020},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
    author = {Vora, Sourabh and Lang, Alex H and Helou, Bassam and Beijbom, Oscar},
    pages = {4604--4612}
}

@inproceedings{Lang2019a,
    title = {{Pointpillars: Fast encoders for object detection from point clouds}},
    year = {2019},
    booktitle = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
    author = {Lang, Alex H. and Vora, Sourabh and Caesar, Holger and Zhou, Lubing and Yang, Jiong and Beijbom, Oscar},
    pages = {12689--12697},
    volume = {2019-June},
    isbn = {9781728132938},
    doi = {10.1109/CVPR.2019.01298},
    issn = {10636919},
    arxivId = {1812.05784},
    keywords = {3D from Multiview and Sensors, Deep Learning, Robotics + Driving, Scene Analysis and Understanding, Vision Applications}
}

@inproceedings{Shi2019,
    title = {{Pointrcnn: 3d object proposal generation and detection from point cloud}},
    year = {2019},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
    author = {Shi, Shaoshuai and Wang, Xiaogang and Li, Hongsheng},
    pages = {770--779}
}

@inproceedings{Papernot2017b,
    title = {{Practical black-box attacks against machine learning}},
    year = {2017},
    booktitle = {ASIA CCS 2017 - Proceedings of the 2017 ACM Asia Conference on Computer and Communications Security},
    author = {Papernot, Nicolas and McDaniel, Patrick and Goodfellow, Ian and Jha, Somesh and Celik, Z. Berkay and Swami, Ananthram},
    pages = {506--519},
    isbn = {9781450349444},
    doi = {10.1145/3052973.3053009},
    arxivId = {1602.02697}
}

@article{Orekondy2019,
    title = {{Prediction poisoning: Utility-constrained defenses against model stealing attacks}},
    year = {2019},
    journal = {arXiv},
    author = {Orekondy, Tribhuvanesh and Schiele, Bernt and Fritz, Mario},
    issn = {23318422}
}

@inproceedings{Wang2019b,
    title = {{Pseudo-LiDAR from visual depth estimation: Bridging the gap in 3D object detection for autonomous driving}},
    year = {2018},
    booktitle = {arXiv},
    author = {Wang, Yan and Chao, Wei Lun and Garg, Divyansh and Hariharan, Bharath and Campbell, Mark and Weinberger, Kilian Q.},
    pages = {8445--8453},
    issn = {23318422}
}

@inproceedings{Shoukry2015c,
    title = {{PyCRA: Physical challenge-response authentication for active sensors under spoofing attacks}},
    year = {2015},
    booktitle = {Proceedings of the ACM Conference on Computer and Communications Security},
    author = {Shoukry, Yasser and Martin, Paul and Yona, Yair and Diggavi, Suhas and Srivastava, Mani},
    pages = {1004--1015},
    volume = {2015-Octob},
    isbn = {9781450338325},
    doi = {10.1145/2810103.2813679},
    issn = {15437221},
    keywords = {Active sensors, Challenge-response authentication, Embedded Security, Physical attacks, Spoofing attacks}
}

@article{Kwon2017a,
    title = {{Reachability analysis for safety assurance of cyber-physical systems against cyber attacks}},
    year = {2018},
    journal = {IEEE Transactions on Automatic Control},
    author = {Kwon, Cheolhyeon and Hwang, Inseok},
    number = {7},
    pages = {2272--2279},
    volume = {63},
    publisher = {IEEE},
    doi = {10.1109/TAC.2017.2761762},
    issn = {00189286},
    keywords = {Cyber attack, cyber-physical system (CPS), estimation, fault detection, linear systems}
}

@article{Venkataraman2019b,
    title = {{Recovering robustness in model-free reinforcement learning}},
    year = {2019},
    journal = {Proceedings of the American Control Conference},
    author = {Venkataraman, Harish K. and Seiler, Peter J.},
    number = {Section IV},
    pages = {4210--4216},
    volume = {2019-July},
    isbn = {9781538679265},
    doi = {10.23919/acc.2019.8815368},
    issn = {07431619},
    arxivId = {1810.09337}
}

@book{Sutton2018,
    title = {{Reinforcement learning: An introduction}},
    year = {2018},
    author = {Sutton, Richard S and Barto, Andrew G},
    publisher = {MIT press},
    isbn = {0262352702}
}

@article{Jovanov2019b,
    title = {{Relaxing Integrity Requirements for Attack-Resilient Cyber-Physical Systems}},
    year = {2019},
    journal = {IEEE Transactions on Automatic Control},
    author = {Jovanov, Ilija and Pajic, Miroslav},
    number = {12},
    pages = {4843--4858},
    volume = {64},
    doi = {10.1109/TAC.2019.2898510},
    issn = {15582523},
    arxivId = {1707.02950},
    keywords = {Attack detection, Kalman filtering, attack-resilient state estimation, cyber-physical systems (CPS) security, linear systems}
}

@article{Petit2015c,
    title = {{Remote Attacks on Automated Vehicles Sensors: Experiments on Camera and LiDAR}},
    year = {2015},
    journal = {Blackhat.com},
    author = {Petit, Jonathan; and Stottelaar, Bas and Feiri, Michael and Kargl, Frank},
    pages = {1--13},
    volume = {11},
    url = {https://www.blackhat.com/docs/eu-15/materials/eu-15-Petit-Self-Driving-And-Connected-Cars-Fooling-Sensors-And-Tracking-Drivers-wp1.pdf},
    keywords = {automated vehicle, camera, lidar, remote attack, security}
}

@inproceedings{Tsai2020,
    title = {{Robust Adversarial Objects against Deep Learning Models}},
    year = {2020},
    booktitle = {Proceedings of the AAAI Conference on Artificial Intelligence},
    author = {Tsai, Tzungyu and Yang, Kaichen and Ho, Tsung-Yi and Jin, Yier},
    number = {01},
    pages = {954--962},
    volume = {34},
    isbn = {2374-3468},
    doi = {10.1609/aaai.v34i01.5443},
    issn = {2159-5399}
}

@article{Li2018,
    title = {{Robust adversarial perturbation on deep proposal-based models}},
    year = {2018},
    journal = {arXiv},
    author = {Li, Yuezun and Tian, Daniel and Chang, Mingching and Bian, Xiao and Lyu, Siwei},
    issn = {23318422},
    arxivId = {1809.05962}
}

@inproceedings{Eykholt2018b,
    title = {{Robust Physical-World Attacks on Deep Learning Visual Classification}},
    year = {2018},
    booktitle = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
    author = {Eykholt, Kevin and Evtimov, Ivan and Fernandes, Earlence and Li, Bo and Rahmati, Amir and Xiao, Chaowei and Prakash, Atul and Kohno, Tadayoshi and Song, Dawn},
    pages = {1625--1634},
    isbn = {9781538664209},
    doi = {10.1109/CVPR.2018.00175},
    issn = {10636919}
}

@inproceedings{Dong2020b,
    title = {{Robust Superpixel-Guided Attentional Adversarial Attack}},
    year = {2020},
    booktitle = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
    author = {Dong, Xiaoyi and Han, Jiangfan and Chen, Dongdong and Liu, Jiayang and Bian, Huanyu and Ma, Zehua and Li, Hongsheng and Wang, Xiaogang and Zhang, Weiming and Yu, Nenghai},
    pages = {12892--12901},
    doi = {10.1109/CVPR42600.2020.01291},
    issn = {10636919}
}

@inproceedings{Wicker2019,
    title = {{Robustness of 3D Deep Learning in an Adversarial Setting}},
    year = {2019},
    booktitle = {arXiv},
    author = {Wicker, Matthew and Kwiatkowska, Marta},
    pages = {11767--11775},
    issn = {23318422}
}

@inproceedings{Pajic2014b,
    title = {{Robustness of attack-resilient state estimators}},
    year = {2014},
    booktitle = {2014 ACM/IEEE International Conference on Cyber-Physical Systems, ICCPS 2014},
    author = {Pajic, Miroslav and Weimer, James and Bezzo, Nicola and Tabuada, Paulo and Sokolsky, Oleg and Lee, Insup and Pappas, George J.},
    pages = {163--174},
    publisher = {IEEE},
    isbn = {9781479949311},
    doi = {10.1109/ICCPS.2014.6843720}
}

@article{Doyle1979b,
    title = {{Robustness with Observers}},
    year = {1979},
    journal = {IEEE Transactions on Automatic Control},
    author = {Doyle, J. C. and Stein, G.},
    number = {4},
    pages = {607--611},
    volume = {24},
    doi = {10.1109/TAC.1979.1102095},
    issn = {15582523},
    keywords = {Control systems, Filtering theory, Linear feedback control systems, Linear systems, Observers, Robust control, Robust stability, Robustness, State feedback, Student members, Transfer functions, time-invariant continuous-time}
}

@inproceedings{Munos2016b,
    title = {{Safe and efficient off-policy reinforcement learning}},
    year = {2016},
    booktitle = {Advances in Neural Information Processing Systems},
    author = {Munos, Rémi and Stepleton, Thomas and Harutyunyan, Anna and Bellemare, Marc G.},
    pages = {1054--1062},
    issn = {10495258},
    arxivId = {1606.02647}
}

@inproceedings{Amin2009a,
    title = {{Safe and secure networked control systems under denial-of-service attacks}},
    year = {2009},
    booktitle = {Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
    author = {Amin, Saurabh and C{\'{a}}rdenas, Alvaro A. and Sastry, S. Shankar},
    pages = {31--45},
    volume = {5469},
    publisher = {Springer},
    isbn = {9783642006012},
    doi = {10.1007/978-3-642-00602-9{\_}3},
    issn = {03029743}
}

@article{Berkenkamp2017a,
    title = {{Safe model-based reinforcement learning with stability guarantees}},
    year = {2017},
    journal = {arXiv},
    author = {Berkenkamp, Felix and Turchetta, Matteo and Schoellig, Angela P. and Krause, Andreas},
    issn = {23318422}
}

@inproceedings{Sun2020g,
    title = {{Scalability in perception for autonomous driving: Waymo open dataset}},
    year = {2019},
    booktitle = {arXiv},
    author = {Sun, Pei and Kretzschmar, Henrik and Dotiwalla, Xerxes and Chouard, Aurélien and Patnaik, Vijaysai and Tsui, Paul and Guo, James and Zhou, Yin and Chai, Yuning and Caine, Benjamin and Vasudevan, Vijay and Han, Wei and Ngiam, Jiquan and Zhao, Hang and Timofeev, Aleksei and Ettinger, Scott and Krivokon, Maxim and Gao, Amy and Joshi, Aditya and Zhang, Yu and Shlens, Jonathon and Chen, Zhifeng and Anguelov, Dragomir},
    pages = {2446--2454},
    issn = {23318422}
}

@inproceedings{Eysenbach2019b,
    title = {{Search on the Replay Buffer: Bridging Planning and Reinforcement Learning}},
    year = {2019},
    booktitle = {arXiv},
    author = {Eysenbach, Benjamin and Salakhutdinov, Ruslan and Levine, Sergey},
    pages = {15246--15257},
    issn = {23318422},
    arxivId = {1906.05253}
}

@article{Fawzi2014b,
    title = {{Secure estimation for cyber-physical systems under adversarial actuator attacks}},
    year = {2017},
    journal = {IET Control Theory and Applications},
    author = {Xie, Chun Hua and Yang, Guang Hong},
    number = {17},
    pages = {2939--2946},
    volume = {11},
    publisher = {IEEE},
    doi = {10.1049/iet-cta.2017.0561},
    issn = {17518652}
}

@inproceedings{Fawzi2011a,
    title = {{Secure state-estimation for dynamical systems under active adversaries}},
    year = {2011},
    booktitle = {2011 49th Annual Allerton Conference on Communication, Control, and Computing, Allerton 2011},
    author = {Fawzi, Hamza and Tabuada, Paulo and Diggavi, Suhas},
    pages = {337--344},
    publisher = {IEEE},
    isbn = {9781457718168},
    doi = {10.1109/Allerton.2011.6120187}
}

@inproceedings{Mohassel2017,
    title = {{Secureml: A system for scalable privacy-preserving machine learning}},
    year = {2017},
    booktitle = {2017 IEEE Symposium on Security and Privacy (SP)},
    author = {Mohassel, Payman and Zhang, Yupeng},
    pages = {19--38},
    publisher = {IEEE},
    isbn = {1509055339}
}

@inproceedings{Dong2020a,
    title = {{Self-Robust 3D Point Recognition via Gather-Vector Guidance}},
    year = {2020},
    booktitle = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
    author = {Dong, Xiaoyi and Chen, Dongdong and Zhou, Hang and Hua, Gang and Zhang, Weiming and Yu, Nenghai},
    pages = {11513--11521},
    publisher = {IEEE},
    isbn = {1728171687},
    doi = {10.1109/CVPR42600.2020.01153},
    issn = {10636919}
}

@inproceedings{Kocic2018,
    title = {{Sensors and sensor fusion in autonomous vehicles}},
    year = {2018},
    booktitle = {2018 26th Telecommunications Forum (TELFOR)},
    author = {Koci{\'{c}}, Jelena and Jovi{\v{c}}i{\'{c}}, Nenad and Drndarevi{\'{c}}, Vujo},
    pages = {420--425},
    publisher = {IEEE},
    isbn = {1538671719}
}

@inproceedings{Guo2019b,
    title = {{Simple black-box adversarial attacks}},
    year = {2019},
    booktitle = {International Conference on Machine Learning},
    author = {Guo, Chuan and Gardner, Jacob and You, Yurong and Wilson, Andrew Gordon and Weinberger, Kilian},
    pages = {2484--2493},
    publisher = {PMLR},
    isbn = {2640-3498}
}

@inproceedings{Liu2019a,
    title = {{Soft rasterizer: A differentiable renderer for image-based 3d reasoning}},
    year = {2019},
    booktitle = {arXiv},
    author = {Liu, Shichen and Li, Tianye and Chen, Weikai and Li, Hao},
    pages = {7708--7717},
    issn = {23318422}
}

@inproceedings{Zhu2011a,
    title = {{Stackelberg-game analysis of correlated attacks in cyber-physical systems}},
    year = {2011},
    booktitle = {Proceedings of the American Control Conference},
    author = {Zhu, Minghui and Mart{\'{i}}nez, Sonia},
    pages = {4063--4068},
    publisher = {IEEE},
    isbn = {9781457700804},
    doi = {10.1109/acc.2011.5991463},
    issn = {07431619}
}

@article{Hu2018a,
    title = {{State estimation under false data injection attacks: Security analysis and system protection}},
    year = {2018},
    journal = {Automatica},
    author = {Hu, Liang and Wang, Zidong and Han, Qing Long and Liu, Xiaohui},
    pages = {176--183},
    volume = {87},
    publisher = {Elsevier},
    doi = {10.1016/j.automatica.2017.09.028},
    issn = {00051098},
    keywords = {False data injection attacks, Networked control systems, Security analysis, State estimation}
}

@inproceedings{Tramer2016,
    title = {{Stealing machine learning models via prediction APIs}},
    year = {2016},
    booktitle = {Proceedings of the 25th USENIX Security Symposium},
    author = {Tram{\`{e}}r, Florian and Zhang, Fan and Juels, Ari and Reiter, Michael K. and Ristenpart, Thomas},
    pages = {601--618},
    isbn = {9781931971324},
    arxivId = {1609.02943}
}

@inproceedings{Dan2010a,
    title = {{Stealth attacks and protection schemes for state estimators in power systems}},
    year = {2010},
    booktitle = {2010 1st IEEE International Conference on Smart Grid Communications, SmartGridComm 2010},
    author = {D{\'{a}}n, György and Sandberg, Henrik},
    pages = {1--6},
    publisher = {IEEE},
    isbn = {9781424465125},
    doi = {10.1109/smartgrid.2010.5622046}
}

@inproceedings{Amin2010a,
    title = {{Stealthy deception attacks on water SCADA systems}},
    year = {2010},
    booktitle = {HSCC'10 - Proceedings of the 13th ACM International Conference on Hybrid Systems: Computation and Control},
    author = {Amin, Saurabh and Litrico, Xavier and Sastry, S. Shankar and Bayen, Alexandre M.},
    pages = {161--170},
    isbn = {9781605589558},
    doi = {10.1145/1755952.1755976},
    keywords = {Secure control systems, Switching PDEs, Water mangement}
}

@article{Langner2011b,
    title = {{Stuxnet: Dissecting a cyberwarfare weapon}},
    year = {2011},
    journal = {IEEE Security and Privacy},
    author = {Langner, Ralph},
    number = {3},
    pages = {49--51},
    volume = {9},
    publisher = {IEEE},
    doi = {10.1109/MSP.2011.67},
    issn = {15407993},
    keywords = {Ralph Langner, SCADA, Stuxnet, cyberwarfare, digital code signing}
}

@article{Li2003,
    title = {{Survey of maneuvering target tracking. Part I. Dynamic models}},
    year = {2003},
    journal = {IEEE Transactions on aerospace and electronic systems},
    author = {Li, X Rong and Jilkov, Vesselin P},
    number = {4},
    pages = {1333--1364},
    volume = {39},
    publisher = {IEEE},
    issn = {0018-9251}
}

@article{Li2010,
    title = {{Survey of maneuvering target tracking. Part II: Motion models of ballistic and space targets}},
    year = {2010},
    journal = {IEEE Transactions on Aerospace and Electronic Systems},
    author = {Li, X Rong and Jilkov, Vesselin P},
    number = {1},
    pages = {96--119},
    volume = {46},
    publisher = {IEEE},
    issn = {0018-9251}
}

@article{Li2005,
    title = {{Survey of maneuvering target tracking. Part V. Multiple-model methods}},
    year = {2005},
    journal = {IEEE Transactions on Aerospace and Electronic Systems},
    author = {Li, X Rong and Jilkov, Vesselin P},
    number = {4},
    pages = {1255--1321},
    volume = {41},
    publisher = {IEEE},
    issn = {0018-9251}
}

@inproceedings{Li2001,
    title = {{Survey of maneuvering target tracking: III. Measurement models}},
    year = {2001},
    booktitle = {Signal and Data Processing of Small Targets 2001},
    author = {Li, X Rong and Jilkov, Vesselin P},
    pages = {423--446},
    volume = {4473},
    publisher = {International Society for Optics and Photonics}
}

@inproceedings{Athalye2018d,
    title = {{Synthesizing robust adversarial examples}},
    year = {2017},
    booktitle = {arXiv},
    author = {Athalye, Anish and Engstrom, Logan and Ilyas, Andrew and Kwok, Kevin},
    pages = {284--293},
    publisher = {PMLR},
    isbn = {2640-3498},
    issn = {23318422}
}

@book{Hastie2009,
    title = {{The Elements of Statistical Learning: Data Mining, Inference, and Prediction}},
    year = {2004},
    booktitle = {Journal of the American Statistical Association},
    author = {Ruppert, David},
    number = {466},
    pages = {567--567},
    volume = {99},
    publisher = {Springer Science {\&} Business Media},
    isbn = {0387848584},
    doi = {10.1198/jasa.2004.s339},
    issn = {0162-1459}
}

@inproceedings{Papernot2016c,
    title = {{The limitations of deep learning in adversarial settings}},
    year = {2016},
    booktitle = {Proceedings - 2016 IEEE European Symposium on Security and Privacy, EURO S and P 2016},
    author = {Papernot, Nicolas and Mcdaniel, Patrick and Jha, Somesh and Fredrikson, Matt and Celik, Z. Berkay and Swami, Ananthram},
    pages = {372--387},
    publisher = {IEEE},
    isbn = {9781509017515},
    doi = {10.1109/EuroSP.2016.36},
    arxivId = {1511.07528}
}

@inproceedings{Slay2007a,
    title = {{The liturgical forensic examination: Tracing activity on a windows-based desktop}},
    year = {2002},
    booktitle = {Cyber Forensics: A Field Manual for Collecting, Examining, and Preserving Evidence of Computer Crimes},
    author = {Greenfield, Robert S.},
    pages = {47--78},
    publisher = {Springer},
    isbn = {9781420000115},
    doi = {10.1201/9781420000115}
}

@article{Richards2018a,
    title = {{The lyapunov neural network: Adaptive stability certification for safe learning of dynamical systems}},
    year = {2018},
    journal = {arXiv},
    author = {Richards, Spencer M. and Berkenkamp, Felix and Krause, Andreas},
    issn = {23318422},
    arxivId = {1808.00924},
    keywords = {Lyapunov stability, Reinforcement learning, Safe learning}
}

@article{Everingham2010,
    title = {{The pascal visual object classes (voc) challenge}},
    year = {2010},
    journal = {International journal of computer vision},
    author = {Everingham, Mark and Van Gool, Luc and Williams, Christopher K I and Winn, John and Zisserman, Andrew},
    number = {2},
    pages = {303--338},
    volume = {88},
    publisher = {Springer},
    issn = {1573-1405}
}

@article{Mobasher2007b,
    title = {{Toward trustworthy recommender systems: An analysis of attack models and algorithm robustness}},
    year = {2007},
    journal = {ACM Transactions on Internet Technology},
    author = {Mobasher, Bamshad and Burke, Robin and Bhaumik, Runa and Williams, Chad},
    number = {4},
    pages = {23-es},
    volume = {7},
    publisher = {ACM New York, NY, USA},
    doi = {10.1145/1278366.1278372},
    issn = {15335399},
    keywords = {Attack detection, Collaborative filtering, Profile injection attacks, Recommender systems, Shilling}
}

@article{Madry2017b,
    title = {{Towards deep learning models resistant to adversarial attacks}},
    year = {2017},
    journal = {International Conference on Learning Representations},
    author = {M{\c{a}}dry, Aleksander and Makelov, Aleksandar and Schmidt, Ludwig and Tsipras, Dimitris and Vladu, Adrian},
    issn = {23318422},
    arxivId = {1706.06083}
}

@inproceedings{Carlini2017d,
    title = {{Towards Evaluating the Robustness of Neural Networks}},
    year = {2017},
    booktitle = {Proceedings - IEEE Symposium on Security and Privacy},
    author = {Carlini, Nicholas and Wagner, David},
    pages = {39--57},
    publisher = {IEEE},
    isbn = {9781509055326},
    doi = {10.1109/SP.2017.49},
    issn = {10816011},
    arxivId = {1608.04644}
}

@inproceedings{Sun2020h,
    title = {{Towards robust LiDAR-based perception in autonomous driving: General black-box adversarial sensor attack and countermeasures}},
    year = {2020},
    booktitle = {Proceedings of the 29th USENIX Security Symposium},
    author = {Sun, Jiachen and Cao, Yulong and Chen, Qi Alfred and Morley Mao, Z.},
    pages = {877--894},
    url = {http://arxiv.org/abs/2006.16974},
    isbn = {9781939133175},
    arxivId = {2006.16974}
}

@article{Wang2020a,
    title = {{Towards robust sensor fusion in visual perception}},
    year = {2020},
    journal = {arXiv},
    author = {Wang, Shaojie and Wu, Tong and Vorobeychik, Yevgeniy},
    issn = {23318422},
    arxivId = {2006.13192},
    keywords = {Adversarial attacks, Autonomous driving, Robust sensor fusion}
}

@article{Abdelfattah2021a,
    title = {{Towards Universal Physical Attacks On Cascaded Camera-Lidar 3D Object Detection Models}},
    year = {2021},
    journal = {arXiv preprint arXiv:2101.10747},
    author = {Abdelfattah, Mazen and Yuan, Kaiwen and Wang, Z Jane and Ward, Rabab}
}

@article{Wei2018,
    title = {{Transferable Adversarial Attacks for Image and Video Object Detection}},
    year = {2018},
    journal = {arXiv},
    author = {Wei, Xingxing and Liang, Siyuan and Chen, Ning and Cao, Xiaochun},
    issn = {23318422}
}

@inproceedings{Tunga2018a,
    title = {{Tuning windowed chi-squared detectors for sensor attacks}},
    year = {2017},
    booktitle = {arXiv},
    author = {Tunga, R. and Murguia, Carlos and Ruths, Justin},
    pages = {1752--1757},
    publisher = {IEEE},
    isbn = {1538654288},
    issn = {23318422}
}

@book{Shalev-Shwartz2014a,
    title = {{Understanding machine learning: From theory to algorithms}},
    year = {2013},
    booktitle = {Understanding Machine Learning: From Theory to Algorithms},
    author = {Shalev-Shwartz, Shai and Ben-David, Shai},
    pages = {1--397},
    volume = {9781107057},
    publisher = {Cambridge university press},
    isbn = {9781107298019},
    doi = {10.1017/CBO9781107298019}
}

@article{Kerns2014a,
    title = {{Unmanned Aircraft Capture and Control Via GPS Spoofing. Journal of Field Robotics}},
    year = {2014},
    journal = {Journal of Field Robotics},
    author = {J.Kerns, Andrew and P.Shepard, Daniel and A.Bhatti, Jahshan and E.Humphreys, Todd},
    number = {4},
    pages = {617--636},
    volume = {31},
    publisher = {Wiley Online Library},
    isbn = {9783000248832},
    issn = {1556-4959},
    keywords = {ATC, Cramer-Rao lower bound, Minimum mean-squared error (MMSE), Quantized measurement, State estimation, Tracking}
}

@article{Li2016a,
    title = {{Vehicle detection from 3D lidar using fully convolutional network}},
    year = {2016},
    journal = {Robotics: Science and Systems},
    author = {Li, Bo and Zhang, Tianlei and Xia, Tian},
    volume = {12},
    isbn = {9780992374723},
    doi = {10.15607/rss.2016.xii.042},
    issn = {2330765X},
    arxivId = {1608.07916}
}

@article{Geiger2013b,
    title = {{Vision meets robotics: The KITTI dataset}},
    year = {2013},
    journal = {International Journal of Robotics Research},
    author = {Geiger, A. and Lenz, P. and Stiller, C. and Urtasun, R.},
    number = {11},
    pages = {1231--1237},
    volume = {32},
    publisher = {Sage Publications Sage UK: London, England},
    doi = {10.1177/0278364913491297},
    issn = {02783649},
    keywords = {Dataset, GPS, KITTI, SLAM, autonomous driving, benchmarks, cameras, computer vision, field robotics, laser, mobile robotics, object detection, optical flow, stereo, tracking}
}

@article{Mehta2017,
    title = {{Vnect: Real-time 3d human pose estimation with a single rgb camera}},
    year = {2017},
    journal = {ACM Transactions on Graphics (TOG)},
    author = {Mehta, Dushyant and Sridhar, Srinath and Sotnychenko, Oleksandr and Rhodin, Helge and Shafiei, Mohammad and Seidel, Hans-Peter and Xu, Weipeng and Casas, Dan and Theobalt, Christian},
    number = {4},
    pages = {1--14},
    volume = {36},
    publisher = {ACM New York, NY, USA},
    issn = {0730-0301}
}

@inproceedings{Zhou2018a,
    title = {{VoxelNet: End-to-End Learning for Point Cloud Based 3D Object Detection}},
    year = {2018},
    booktitle = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
    author = {Zhou, Yin and Tuzel, Oncel},
    pages = {4490--4499},
    isbn = {9781538664209},
    doi = {10.1109/CVPR.2018.00472},
    issn = {10636919},
    arxivId = {1711.06396}
}

@article{Weng3DMetrics,
    title = {{3D Multi-Object Tracking: A Baseline and New Evaluation Metrics}},
    author = {Weng, Xinshuo and Wang, Jianren and Held, David and Kitani, Kris},
    url = {http://www.},
    isbn = {9781728162119}
}

@article{Weng2019ATracking,
    title = {{A baseline for 3d multi-object tracking}},
    year = {2019},
    journal = {arXiv preprint arXiv:1907.03961},
    author = {Weng, Xinshuo and Kitani, Kris},
    number = {2},
    pages = {6},
    volume = {1}
}

@inproceedings{Du2018AVehicles,
    title = {{A general pipeline for 3d detection of vehicles}},
    year = {2018},
    booktitle = {2018 IEEE International Conference on Robotics and Automation (ICRA)},
    author = {Du, Xinxin and Ang, Marcelo H and Karaman, Sertac and Rus, Daniela},
    pages = {3194--3200},
    publisher = {IEEE},
    isbn = {1538630818}
}

@article{Giusti2016ARobots,
    title = {{A Machine Learning Approach to Visual Perception of Forest Trails for Mobile Robots}},
    year = {2016},
    journal = {IEEE Robotics and Automation Letters},
    author = {Giusti, Alessandro and Guzzi, Jerome and Ciresan, Dan C. and He, Fang Lin and Rodriguez, Juan P. and Fontana, Flavio and Faessler, Matthias and Forster, Christian and Schmidhuber, Jurgen and Caro, Gianni Di and Scaramuzza, Davide and Gambardella, Luca M.},
    number = {2},
    month = {7},
    pages = {661--667},
    volume = {1},
    publisher = {Institute of Electrical and Electronics Engineers Inc.},
    doi = {10.1109/LRA.2015.2509024},
    issn = {23773766},
    keywords = {Aerial Robotics, Deep Learning, Machine Learning, Visual-Based Navigation}
}

@article{MaleyAAnalysis,
    title = {{A Modular Approach to Kalman Filter Design and Analysis}},
    author = {Maley, James},
    keywords = {ARL-TR-9165, DEVCOM ARL, Kalman filtering, navigation, state estimation}
}

@article{SunANavigation,
    title = {{A new variational Bayesian adaptive extended Kalman filter for cooperative navigation}},
    journal = {mdpi.com},
    author = {Sun, C and Zhang, Y and Wang, G and Sensors, W Gao - and 2018, undefined},
    url = {https://www.mdpi.com/323464},
    doi = {10.3390/s18082538},
    keywords = {cooperative navigation, extended Kalman filter (EKF), nonlinear filters, variational Bayesian}
}

@article{HuangAMatrices,
    title = {{A novel adaptive Kalman filter with inaccurate process and measurement noise covariance matrices}},
    journal = {ieeexplore.ieee.org},
    author = {Huang, Y and Zhang, Y and Wu, Z and {\ldots}, N Li - IEEE Transactions on and 2017, undefined},
    url = {https://ieeexplore.ieee.org/abstract/document/8025799/}
}

@inproceedings{Ma2019AccurateDriving,
    title = {{Accurate monocular 3d object detection via color-embedded 3d reconstruction for autonomous driving}},
    year = {2019},
    booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision},
    author = {Ma, Xinzhu and Wang, Zhihui and Li, Haojie and Zhang, Pengbo and Ouyang, Wanli and Fan, Xin},
    pages = {6851--6860}
}

@article{Koren2018AdaptiveVehicles,
    title = {{Adaptive Stress Testing for Autonomous Vehicles}},
    year = {2018},
    journal = {IEEE Intelligent Vehicles Symposium, Proceedings},
    author = {Koren, Mark and Alsaif, Saud and Lee, Ritchie and Kochenderfer, Mykel J.},
    month = {10},
    pages = {1898--1904},
    volume = {2018-June},
    publisher = {Institute of Electrical and Electronics Engineers Inc.},
    isbn = {9781538644522},
    doi = {10.1109/IVS.2018.8500400},
    arxivId = {1902.01909}
}

@article{WangAdversarialModels,
    title = {{Adversarial Robustness of Deep Sensor Fusion Models}},
    author = {Wang, Shaojie and Wu, Tong and Chakrabarti, Ayan and Vorobeychik, Yevgeniy},
    arxivId = {2006.13192v2}
}

@article{Cao2021AutomatedTargets,
    title = {{Automated Tracking System For LiDAR Spoofing Attacks On Moving Targets}},
    year = {2021},
    author = {Cao, Yulong and Ma, Jiaxiang and Fu, Kevin and Sara, Rampazzi and Mao, Morley}
}

@article{Cao2021AutomatedTargetsb,
    title = {{Automated Tracking System For LiDAR Spoofing Attacks On Moving Targets}},
    year = {2021},
    author = {Cao, Yulong and Ma, Jiaxiang and Fu, Kevin and Sara, Rampazzi and Mao, Morley}
}

@inproceedings{Kato2018AutowareSystems,
    title = {{Autoware on board: Enabling autonomous vehicles with embedded systems}},
    year = {2018},
    booktitle = {2018 ACM/IEEE 9th International Conference on Cyber-Physical Systems (ICCPS)},
    author = {Kato, Shinpei and Tokunaga, Shota and Maruyama, Yuya and Maeda, Seiya and Hirabayashi, Manato and Kitsukawa, Yuki and Monrroy, Abraham and Ando, Tomohito and Fujii, Yusuke and Azumi, Takuya},
    pages = {287--296},
    publisher = {IEEE},
    isbn = {153865301X}
}

@inproceedings{Du2017CarFramework,
    title = {{Car detection for autonomous vehicle: LIDAR and vision fusion approach through deep learning framework}},
    year = {2017},
    booktitle = {2017 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
    author = {Du, Xinxin and Ang, Marcelo H and Rus, Daniela},
    pages = {749--754},
    publisher = {IEEE},
    isbn = {1538626829}
}

@article{YinCenter-basedTracking,
    title = {{Center-based 3D Object Detection and Tracking}},
    author = {Yin, Tianwei and Zhou, Xingyi and Kr{\"{a}}henb{\"{u}}hl, Philipp},
    url = {https://github.com/tianweiy/CenterPoint.}
}

@article{SimonComplex-YOLO:Clouds,
    title = {{Complex-YOLO: An Euler-Region-Proposal for Real-time 3D Object Detection on Point Clouds}},
    author = {Simon, Martin and Milz, Stefan and Amende, Karl and Gross, Horst-Michael},
    keywords = {3D Object Detection, Au-tonomous Driving, Lidar, Point Cloud Processing}
}

@article{LillicrapCONTINUOUSLEARNING,
    title = {{CONTINUOUS CONTROL WITH DEEP REINFORCEMENT LEARNING}},
    author = {Lillicrap, Timothy P and Hunt, Jonathan J and Pritzel, Alexander and Heess, Nicolas and Erez, Tom and Tassa, Yuval and Silver, David and Wierstra, Daan},
    url = {https://goo.gl/J4PIAz},
    arxivId = {1509.02971v6}
}

@article{Vivek2019CyberphysicalVehicles,
    title = {{Cyberphysical risks of hacked internet-connected vehicles}},
    year = {2019},
    journal = {Physical Review E},
    author = {Vivek, Skanda and Yanni, David and Yunker, Peter J and Silverberg, Jesse L},
    number = {1},
    pages = {12316},
    volume = {100},
    publisher = {APS}
}

@article{Lotter2016DeepLearning,
    title = {{Deep predictive coding networks for video prediction and unsupervised learning}},
    year = {2016},
    journal = {arXiv preprint arXiv:1605.08104},
    author = {Lotter, William and Kreiman, Gabriel and Cox, David}
}

@article{CaoDemo:Targets,
    title = {{Demo: Automated Tracking System For LiDAR Spoofing Attacks On Moving Targets}},
    author = {Cao, Yulong and Ma, Jiaxiang and Fu, Kevin and Sara, Rampazzi and Mao, Morley},
    url = {https://dx.doi.org/10.14722/autosec.2021.23019},
    isbn = {1891562681},
    doi = {10.14722/autosec.2021.23019}
}

@article{SilverDeterministicAlgorithms,
    title = {{Deterministic Policy Gradient Algorithms}},
    author = {Silver, David and Heess, Nicolas and Degris, Thomas and Wierstra, Daan and Riedmiller, Martin}
}

@inproceedings{Shen2020DriftSpoofing,
    title = {{Drift with devil: Security of multi-sensor fusion based localization in high-level autonomous driving under GPS spoofing}},
    year = {2020},
    booktitle = {29th USENIX Security Symposium},
    author = {Shen, Junjie and Won, Jun Yeon and Chen, Zeyuan and Chen, Qi Alfred},
    pages = {931--948},
    isbn = {1939133173}
}

@article{KimEagerMOT:Fusion,
    title = {{EagerMOT: 3D Multi-Object Tracking via Sensor Fusion}},
    author = {Kim, Aleksandr and Leal-Taix{\'{e}}, Laura},
    url = {https://github.com/aleksandrkim61/EagerMOT},
    arxivId = {2104.14682v1}
}

@article{Bojarski2016EndCars,
    title = {{End to End Learning for Self-Driving Cars}},
    year = {2016},
    author = {Bojarski, Mariusz and Del Testa, Davide and Dworakowski, Daniel and Firner, Bernhard and Flepp, Beat and Goyal, Prasoon and Jackel, Lawrence D. and Monfort, Mathew and Muller, Urs and Zhang, Jiakai and Zhang, Xin and Zhao, Jake and Zieba, Karol},
    url = {http://arxiv.org/abs/1604.07316},
    arxivId = {1604.07316}
}

@inproceedings{Frossard2018End-to-endDetection,
    title = {{End-to-end learning of multi-sensor 3d tracking by detection}},
    year = {2018},
    booktitle = {2018 IEEE international conference on robotics and automation (ICRA)},
    author = {Frossard, Davi and Urtasun, Raquel},
    pages = {635--642},
    publisher = {IEEE},
    isbn = {1538630818}
}

@inproceedings{Huang2020Epnet:Detection,
    title = {{Epnet: Enhancing point features with image semantics for 3d object detection}},
    year = {2020},
    booktitle = {European Conference on Computer Vision},
    author = {Huang, Tengteng and Liu, Zhe and Chen, Xiwu and Bai, Xiang},
    pages = {35--52},
    publisher = {Springer}
}

@article{Bar-Shalom2001EstimationNavigation,
    title = {{Estimation with Applications To Tracking and Navigation}},
    year = {2001},
    author = {Bar-Shalom, Yaakov and Li, X Rong and Kirubarajan, Thiagalingam},
    isbn = {0-471-22127-9}
}

@article{Liu2011FalseGrids,
    title = {{False data injection attacks against state estimation in electric power grids}},
    year = {2011},
    journal = {ACM Trans. Info. Syst. Sec},
    author = {Liu, Y and Ning, P and Reiter, M K},
    pages = {33},
    volume = {14},
    url = {http://doi.acm.org/10.1145/1952982.1952995},
    doi = {10.1145/1952982.1952995},
    keywords = {K65 [Management of Computing and Information Systems]: Security and Protection General Terms: Algorithms, Security Additional Key Words and Phrases: Power grids, attack, state estimation}
}

@article{JiaFOOLINGTRACKING,
    title = {{FOOLING DETECTION ALONE IS NOT ENOUGH: AD-VERSARIAL ATTACK AGAINST MULTIPLE OBJECT TRACKING}},
    author = {Jia, Yunhan and Lu, Yantao and Shen, Junjie and Chen, Qi Alfred and Chen, Hao and Zhong, Zhenyu and Wei, Tao}
}

@article{JiaFOOLINGTRACKINGb,
    title = {{FOOLING DETECTION ALONE IS NOT ENOUGH: AD-VERSARIAL ATTACK AGAINST MULTIPLE OBJECT TRACKING}},
    author = {Jia, Yunhan and Lu, Yantao and Shen, Junjie and Chen, Qi Alfred and Chen, Hao and Zhong, Zhenyu and Wei, Tao}
}

@book{Horst2013GlobalApproaches,
    title = {{Global optimization: Deterministic approaches}},
    year = {2013},
    author = {Horst, Reiner and Tuy, Hoang},
    publisher = {Springer Science {\&} Business Media},
    isbn = {3662025981}
}

@article{Yu2020InvestigatingLearning,
    title = {{Investigating vulnerability to adversarial examples on multimodal data fusion in deep learning}},
    year = {2020},
    journal = {arXiv preprint arXiv:2005.10987},
    author = {Yu, Youngjoon and Lee, Hong Joo and Kim, Byeong Cheon and Kim, Jung Uk and Ro, Yong Man}
}

@inproceedings{Cao2021InvisibleAttacks,
    title = {{Invisible for both Camera and LiDAR: Security of Multi-Sensor Fusion based Perception in Autonomous Driving Under Physical-World Attacks}},
    year = {2021},
    booktitle = {2021 IEEE Symposium on Security and Privacy (SP)},
    author = {Cao, Yulong and Wang, Ningfei and Xiao, Chaowei and Yang, Dawei and Fang, Jin and Yang, Ruigang and Chen, Qi Alfred and Liu, Mingyan and Li, Bo},
    pages = {176--194},
    publisher = {IEEE},
    isbn = {1728189349}
}

@article{Dosovitskiy2017LearningFuture,
    title = {{Learning to act by predicting the future}},
    year = {2017},
    journal = {5th International Conference on Learning Representations, ICLR 2017 - Conference Track Proceedings},
    author = {Dosovitskiy, Alexey and Koltun, Vladlen},
    arxivId = {1611.01779}
}

@article{Mirowski2017LearningEnvironments,
    title = {{Learning to navigate in complex environments}},
    year = {2017},
    journal = {5th International Conference on Learning Representations, ICLR 2017 - Conference Track Proceedings},
    author = {Mirowski, Piotr and Pascanu, Razvan and Viola, Fabio and Soyer, Hubert and Ballard, Andrew J. and Banino, Andrea and Denil, Misha and Goroshin, Ross and Sifre, Laurent and Kavukcuoglu, Koray and Kumaran, Dharshan and Hadsell, Raia},
    url = {https://youtu.be/JL8F82qUG-Q},
    arxivId = {1611.03673}
}

@article{KhazraeiLearning-BasedSystems,
    title = {{Learning-Based Vulnerability Analysis of Cyber-Physical Systems}},
    author = {Khazraei, Amir and Hallyburton, Spencer and Gao, Qitong and Wang, Yu and Pajic, Miroslav},
    arxivId = {2103.06271v2}
}

@inproceedings{Rong2020LgsvlDriving,
    title = {{Lgsvl simulator: A high fidelity simulator for autonomous driving}},
    year = {2020},
    booktitle = {2020 IEEE 23rd International Conference on Intelligent Transportation Systems (ITSC)},
    author = {Rong, Guodong and Shin, Byung Hyun and Tabatabaee, Hadi and Lu, Qiang and Lemke, Steve and Mo{\v{z}}eiko, Mārtiņš and Boise, Eric and Uhm, Geehoon and Gerow, Mark and Mehta, Shalin},
    pages = {1--6},
    publisher = {IEEE},
    isbn = {1728141494}
}

@article{ParkMeasurementData,
    title = {{Measurement noise recommendation for efficient Kalman filtering over a large amount of sensor data}},
    journal = {mdpi.com},
    author = {Park, S and Gil, MS and Im, H and Sensors, YS Moon - and 2019, undefined},
    url = {https://www.mdpi.com/423990},
    doi = {10.3390/s19051168},
    keywords = {denoising autoencoder, filtering accuracy, kalman filtering, measurement noise, sensor data, wavelet transform}
}

@article{MeyerMessageTracking,
    title = {{Message passing algorithms for scalable multitarget tracking}},
    journal = {ieeexplore.ieee.org},
    author = {Meyer, F and Kropfreiter, T and Williams, JL and {\ldots}, R Lau - Proceedings of the and 2018, undefined},
    url = {https://ieeexplore.ieee.org/abstract/document/8290605/}
}

@article{Chang2017MRIMicroarchitecture,
    title = {{MRI assessment of bone structure and microarchitecture}},
    year = {2017},
    journal = {Journal of Magnetic Resonance Imaging},
    author = {Chang, Gregory and Boone, Sean and Martel, Dimitri and Rajapakse, Chamith S. and Hallyburton, Robert S. and Valko, Mitch and Honig, Stephen and Regatte, Ravinder R.},
    number = {2},
    pages = {323--337},
    volume = {46},
    doi = {10.1002/jmri.25647},
    issn = {15222586},
    pmid = {28165650},
    keywords = {bone mineral density (BMD), bone quality, dual-energy x-ray absorptiometry (DXA), finite element analysis (FEA), fragility fractures, osteoporosis}
}

@article{LeCun2005Off-roadLearning,
    title = {{Off-road obstacle avoidance through end-to-end learning}},
    year = {2005},
    journal = {Advances in Neural Information Processing Systems},
    author = {LeCun, Yann and Muller, Urs and Ben, Jan and Cosatto, Eric and Flepp, Beat},
    pages = {739--746},
    url = {http://yann.lecun.com},
    isbn = {9780262232531},
    issn = {10495258}
}

@article{Shalev-Shwartz2017OnCars,
    title = {{On a Formal Model of Safe and Scalable Self-driving Cars}},
    year = {2017},
    author = {Shalev-Shwartz, Shai and Shammah, Shaked and Shashua, Amnon},
    arxivId = {1708.06374v6}
}

@article{ZhangOnVehicles,
    title = {{On Adversarial Robustness of Trajectory Prediction for Autonomous Vehicles}},
    author = {Zhang, Qingzhao and Hu, Shengtuo and Sun, Jiachen and Chen, Qi Alfred and Mao, Z Morley},
    arxivId = {2201.05057v1}
}

@article{GuoOptimalEstimation,
    title = {{Optimal linear cyber-attack on remote state estimation}},
    journal = {ieeexplore.ieee.org},
    author = {Guo, Z and Shi, D and {\ldots}, KH Johansson - IEEE Transactions on and 2016, undefined},
    url = {https://ieeexplore.ieee.org/abstract/document/7470566/?casa_token=HWdGMbXNz1AAAAAA:6ENihV5gyvaHB0biUudf0xg-Pm7pUUJKC1MwZiv4dzUYRcyIZm1byOctlCh8aYm0tmmdJ48JRQ}
}

@inproceedings{Xu2018Pointfusion:Estimation,
    title = {{Pointfusion: Deep sensor fusion for 3d bounding box estimation}},
    year = {2018},
    booktitle = {Proceedings of the IEEE conference on computer vision and pattern recognition},
    author = {Xu, Danfei and Anguelov, Dragomir and Jain, Ashesh},
    pages = {244--253}
}

@article{Ng1999PolicyShaping,
    title = {{Policy invariance under reward transformations: Theory and application to reward shaping}},
    year = {1999},
    journal = {ICML},
    author = {Ng, Andrew Y and Harada, Daishi and Russell, Stuart}
}

@article{Chiu2019ProbabilisticDriving,
    title = {{Probabilistic 3D Multi-Object Tracking for Autonomous Driving}},
    year = {2019},
    journal = {Advances in Neural Information Processing Systems Workshops (NIPS)},
    author = {Chiu, Hsu-kuang and Prioletti, Antonio and Li, Jie and Bohg, Jeannette},
    url = {http://arxiv.org/abs/2001.05673},
    arxivId = {2001.05673}
}

@article{Hu2018ProbabilisticMotion,
    title = {{Probabilistic Prediction of Vehicle Semantic Intention and Motion}},
    year = {2018},
    journal = {IEEE Intelligent Vehicles Symposium, Proceedings},
    author = {Hu, Yeping and Zhan, Wei and Tomizuka, Masayoshi},
    month = {10},
    pages = {307--313},
    volume = {2018-June},
    publisher = {Institute of Electrical and Electronics Engineers Inc.},
    isbn = {9781538644522},
    doi = {10.1109/IVS.2018.8500419},
    arxivId = {1804.03629}
}

@article{BulutProcessFiltering,
    title = {{Process and measurement noise estimation for Kalman filtering}},
    journal = {Springer},
    author = {Bulut, Y and Vines-Cavanaugh, D and Dynamics, D Bernal - Structural and 3, Volume and 2011, undefined},
    url = {https://link.springer.com/chapter/10.1007/978-1-4419-9834-7_36},
    keywords = {Kalman Filter, Measurement Noise NOMENCLATURE, Process Noise}
}

@article{Zhang2017Query-efficientDriving,
    title = {{Query-efficient imitation learning for end-to-end simulated driving}},
    year = {2017},
    journal = {31st AAAI Conference on Artificial Intelligence, AAAI 2017},
    author = {Zhang, Jiakai and Cho, Kyunghyun},
    pages = {2891--2897},
    arxivId = {1605.06450v1}
}

@article{SarkkaRecursiveApproximations,
    title = {{Recursive noise adaptive Kalman filtering by variational Bayesian approximations}},
    journal = {ieeexplore.ieee.org},
    author = {Sarkka, S and Automatic, A Nummenmaa - IEEE Transactions on and 2009, undefined},
    url = {https://ieeexplore.ieee.org/abstract/document/4796261/?casa_token=pgAIyTCBfUYAAAAA:qMRF2CtWBuMMeRRVnRhoFpQseRZQ9KcbBW6u37hZ9dlImGZwmiD0LIVeel65lmPn6QyIsIeDWA}
}

@article{Wiewiora2003ResearchEquivalent,
    title = {{Research Note: Potential-Based Shaping and Q-Value Initialization are Equivalent}},
    year = {2003},
    journal = {Journal of Artificial Intelligence Research},
    author = {Wiewiora, Eric},
    pages = {205--208},
    volume = {19},
    keywords = {Changes and compilation copyright {\textcopyright} The American Association for Artificial Intelligence. All rights reserved., Copyright {\textcopyright} 2003 AI Access}
}

@inproceedings{Guo2018Roboads:Robots,
    title = {{Roboads: Anomaly detection against sensor and actuator misbehaviors in mobile robots}},
    year = {2018},
    booktitle = {2018 48th Annual IEEE/IFIP international conference on dependable systems and networks (DSN)},
    author = {Guo, Pinyao and Kim, Hunmin and Virani, Nurali and Xu, Jun and Zhu, Minghui and Liu, Peng},
    pages = {574--585},
    publisher = {IEEE},
    isbn = {1538655969}
}

@article{Konidaris2012RobotTrees,
    title = {{Robot learning from demonstration by constructing skill trees}},
    year = {2012},
    journal = {International Journal of Robotics Research},
    author = {Konidaris, George and Kuindersma, Scott and Grupen, Roderic and Barto, Andrew},
    number = {3},
    pages = {360--375},
    volume = {31},
    doi = {10.1177/0278364911428653},
    issn = {02783649},
    keywords = {Learning from demonstration, changepoint detection, hierarchical reinforcement learning, motion primitives, motion segmentation}
}

@article{Dean2019RobustControl,
    title = {{Robust Guarantees for Perception-Based Control}},
    year = {2019},
    author = {Dean, Sarah and Matni, Nikolai and Recht, Benjamin and Ye, Vickie},
    url = {http://arxiv.org/abs/1907.03680},
    arxivId = {1907.03680},
    keywords = {Robust control, generalization, learning theory, perception, robotics}
}

@article{LiRTM3D:Driving,
    title = {{RTM3D: Real-time Monocular 3D Detection from Object Keypoints for Autonomous Driving}},
    author = {Li, Peixuan and Zhao, Huaici and Liu, Pengfei and Cao, Feidao},
    url = {https://github.com/Banconxuan/RTM3D.},
    arxivId = {2001.03343v1}
}

@article{TurchettaSafeProcesses,
    title = {{Safe Exploration in Finite Markov Decision Processes with Gaussian Processes}},
    author = {Turchetta, Matteo and Zurich, Eth and Berkenkamp, Felix and Krause, Andreas}
}

@article{LeikeScalableDirection,
    title = {{Scalable agent alignment via reward modeling: a research direction}},
    author = {Leike, Jan and Krueger, David and Everitt, Tom and Martic, Miljan and Vishal, Deepmind and Deepmind, Maini and Deepmind, Shane Legg},
    arxivId = {1811.07871v1}
}

@article{Okelly2019ScalableSimulation,
    title = {{Scalable End-to-End Autonomous Vehicle Testing via Rare-event Simulation}},
    year = {2019},
    author = {O'kelly, Matthew and Sinha, Aman and Namkoong, Hongseok and Duchi, John and Tedrake, Russ},
    arxivId = {1811.00145v3}
}

@article{Hallyburton2021SecurityVehicles,
    title = {{Security Analysis of Camera-LiDAR Semantic-Level Fusion Against Black-Box Attacks on Autonomous Vehicles}},
    year = {2021},
    author = {Hallyburton, R. Spencer and Liu, Yupei and Pajic, Miroslav},
    month = {6},
    url = {http://arxiv.org/abs/2106.07098},
    arxivId = {2106.07098}
}

@article{Deniz2018SegmentationNetworks,
    title = {{Segmentation of the Proximal Femur from MR Images using Deep Convolutional Neural Networks}},
    year = {2018},
    journal = {Scientific Reports},
    author = {Deniz, Cem M. and Xiang, Siyuan and Hallyburton, R. Spencer and Welbeck, Arakua and Babb, James S. and Honig, Stephen and Cho, Kyunghyun and Chang, Gregory},
    number = {1},
    volume = {8},
    doi = {10.1038/s41598-018-34817-6},
    issn = {20452322},
    pmid = {30405145},
    arxivId = {1704.06176}
}

@article{Hau2020Shadow-Catcher:Sensing,
    title = {{Shadow-Catcher: Looking Into Shadows to Detect Ghost Objects in Autonomous Vehicle 3D Sensing}},
    year = {2020},
    journal = {arXiv preprint arXiv:2008.12008},
    author = {Hau, Zhongyuan and Demetriou, Soteris and Mu{\~{n}}oz-Gonz{\'{a}}lez, Luis and Lupu, Emil C.},
    url = {http://arxiv.org/abs/2008.12008},
    arxivId = {2008.12008}
}

@inproceedings{Javdani2015SharedOptimization,
    title = {{Shared autonomy via hindsight optimization}},
    year = {2015},
    booktitle = {Robotics: Science and Systems},
    author = {Javdani, Shervin and Srinivasa, Siddhartha S and Bagnell, J Andrew},
    volume = {11},
    isbn = {9780992374716},
    doi = {10.15607/RSS.2015.XI.032},
    issn = {2330765X},
    arxivId = {1503.07619}
}

@article{Tuncali2018Simulation-basedComponents,
    title = {{Simulation-based Adversarial Test Generation for Autonomous Vehicles with Machine Learning Components}},
    year = {2018},
    journal = {IEEE Intelligent Vehicles Symposium, Proceedings},
    author = {Tuncali, Cumhur Erkan and Fainekos, Georgios and Ito, Hisahiro and Kapinski, James},
    month = {10},
    pages = {1555--1562},
    volume = {2018-June},
    publisher = {Institute of Electrical and Electronics Engineers Inc.},
    isbn = {9781538644522},
    doi = {10.1109/IVS.2018.8500421},
    arxivId = {1804.06760}
}

@article{Roumeliotis2002StochasticMeasurements,
    title = {{Stochastic cloning: A generalized framework for processing relative state measurements}},
    year = {2002},
    journal = {Proceedings - IEEE International Conference on Robotics and Automation},
    author = {Roumeliotis, Stergios I. and Burdick, Joel W.},
    pages = {1788--1795},
    volume = {2},
    doi = {10.1109/ROBOT.2002.1014801},
    issn = {10504729}
}

@article{HeStructureCloud,
    title = {{Structure Aware Single-stage 3D Object Detection from Point Cloud}},
    author = {He, Chenhang and Zeng, Hui and Huang, Jianqiang and Hua, Xian-Sheng and Zhang, Lei}
}

@article{Orzechowski2018TacklingVerification,
    title = {{Tackling Occlusions Limited Sensor Range with Set-based Safety Verification}},
    year = {2018},
    journal = {IEEE Conference on Intelligent Transportation Systems, Proceedings, ITSC},
    author = {Orzechowski, Piotr F. and Meyer, Annika and Lauer, Martin},
    month = {12},
    pages = {1729--1736},
    volume = {2018-November},
    publisher = {Institute of Electrical and Electronics Engineers Inc.},
    isbn = {9781728103235},
    doi = {10.1109/ITSC.2018.8569332},
    arxivId = {1807.01262},
    keywords = {ADAS, automated vehicles, field-of-view, formal verification, occlusions, reachability analysis, risk assessment}
}

@article{Piazzoni2021ViSTA:Vehicles,
    title = {{ViSTA: a Framework for Virtual Scenario-based Testing of Autonomous Vehicles}},
    year = {2021},
    journal = {arXiv preprint arXiv:2109.02529},
    author = {Piazzoni, Andrea and Cherian, Jim and Azhar, Mohamed and Yap, Jing Yew and Shung, James Lee Wei and Vijay, Roshan}
}

@article{Redmon2018Yolov3:Improvement,
    title = {{Yolov3: An incremental improvement}},
    year = {2018},
    journal = {arXiv preprint arXiv:1804.02767},
    author = {Redmon, Joseph and Farhadi, Ali}
}

@inproceedings{Quinonez2020SAVIOR:Invariants,
    title = {{{\{}SAVIOR{\}}: Securing Autonomous Vehicles with Robust Physical Invariants}},
    year = {2020},
    booktitle = {29th {\{}USENIX{\}} Security Symposium ({\{}USENIX{\}} Security 20)},
    author = {Quinonez, Raul and Giraldo, Jairo and Salazar, Luis and Bauman, Erick and Cardenas, Alvaro and Lin, Zhiqiang},
    pages = {895--912},
    isbn = {1939133173}
}
